Sampling Approximately Low-Rank Ising Models: MCMC meets Variational Methods

We consider Ising models on the hypercube with a general interaction matrix $J$, and give a polynomial time sampling algorithm when all but $O(1)$ eigenvalues of $J$ lie in an interval of length one, a situation which occurs in many models of interest. This was previously known for the Glauber dynamics when *all* eigenvalues fit in an interval of length one; however, a single outlier can force the Glauber dynamics to mix torpidly. Our general result implies the first polynomial time sampling algorithms for low-rank Ising models such as Hopfield networks with a fixed number of patterns and Bayesian clustering models with low-dimensional contexts, and greatly improves the polynomial time sampling regime for the antiferromagnetic/ferromagnetic Ising model with inconsistent field on expander graphs. It also improves on previous approximation algorithm results based on the naive mean-field approximation in variational methods and statistical physics. Our approach is based on a new fusion of ideas from the MCMC and variational inference worlds. As part of our algorithm, we define a new nonconvex variational problem which allows us to sample from an exponential reweighting of a distribution by a negative definite quadratic form, and show how to make this procedure provably efficient using stochastic gradient descent. On top of this, we construct a new simulated tempering chain (on an extended state space arising from the Hubbard-Stratonovich transform) which overcomes the obstacle posed by large positive eigenvalues, and combine it with the SGD-based sampler to solve the full problem.

==> colt2022-sample.tex <==
% \documentclass[anon,12pt]{colt2022} % Anonymized submission
% %\documentclass[final,12pt]{colt2022} % Include author names

% % The following packages will be automatically loaded:
% % amsmath, amdssymb, natbib, graphicx, url, algorithm2e

% \title[Short Title]{Full Title of Article}
% \usepackage{times}
% % Use \Name{Author Name} to specify the name.
% % If the surname contains spaces, enclose the surname
% % in braces, e.g. \Name{John {Smith Jones}} similarly
% % if the name has a "von" part, e.g \Name{Jane {de Winter}}.
% % If the first letter in the forenames is a diacritic
% % enclose the diacritic in braces, e.g. \Name{{\'E}louise Smith}

% % Two authors with the same address
% % \coltauthor{\Name{Author Name1} \Email{abc@sample.com}\and
% %  \Name{Author Name2} \Email{xyz@sample.com}\\
% %  \addr Address}

% % Three or more authors with the same address:
% % \coltauthor{\Name{Author Name1} \Email{an1@sample.com}\\
% %  \Name{Author Name2} \Email{an2@sample.com}\\
% %  \Name{Author Name3} \Email{an3@sample.com}\\
% %  \addr Address}

% % Authors with different addresses:
% \coltauthor{%
%  \Name{Author Name1} \Email{abc@sample.com}\\
%  \addr Address 1
%  \AND
%  \Name{Author Name2} \Email{xyz@sample.com}\\
%  \addr Address 2%
% }

% \begin{document}

% \maketitle

% \begin{abstract}%
%   This is a great paper and it has a concise abstract.%
% \end{abstract}

% \begin{keywords}%
%   List of keywords%
% \end{keywords}

% \section{Introduction}

% This is where the content of your paper goes.
% \begin{itemize}
%   \item Limit the main text (not counting references and appendices) to 12 PMLR-formatted pages, using this template. Please add any additional appendix to the same file after references - there is no page limit for the appendix.
%   \item Include, either in the main text or the appendices, \emph{all} details, proofs and derivations required to substantiate the results.
%   \item The contribution, novelty and significance of submissions will be judged primarily based on
% \textit{the main text of 12 pages}. Thus, include enough details, and overview of key arguments, 
% to convince the reviewers of the validity of result statements, and to ease parsing of technical material in the appendix.
%   \item Use the \textbackslash documentclass[anon,12pt]\{colt2022\} option during submission process -- this automatically hides the author names listed under \textbackslash coltauthor. Submissions should NOT include author names or other identifying information in the main text or appendix. To the extent possible, you should avoid including directly identifying information in the text. You should still include all relevant references, discussion, and scientific content, even if this might provide significant hints as to the author identity. But you should generally refer to your own prior work in third person. Do not include acknowledgments in the submission. They can be added in the camera-ready version of accepted papers. 
  
%   Please note that while submissions must be anonymized, and author names are withheld from reviewers, they are known to the area chair overseeing the paper’s review.  The assigned area chair is allowed to reveal author names to a reviewer during the rebuttal period, upon the reviewer’s request, if they deem such information is needed in ensuring a proper review.  
%   \item Use \textbackslash documentclass[final,12pt]\{colt2022\} only during camera-ready submission.
% \end{itemize}



% % Acknowledgments---Will not appear in anonymized version
% \acks{We thank a bunch of people and funding agency.}

% \bibliography{yourbibfile}

% \appendix

% \section{My Proof of Theorem 1}

% This is a boring technical proof.

% \section{My Proof of Theorem 2}

% This is a complete version of a proof sketched in the main text.

% \end{document}


==> formatting.tex <==
\renewcommand{\thesection}{\arabic{section}}

==> macros_colt.tex <==
%LETTERS

%UPPERCASE
\newcommand{\sA}[0]{\mathscr{A}}
\newcommand{\cA}[0]{\mathcal{A}}
\newcommand{\A}[0]{\mathbb{A}}
\newcommand{\cB}[0]{\mathcal{B}}
\newcommand{\C}[0]{\mathbb{C}}
\newcommand{\sC}[0]{\mathcal{C}}%deprecated
\newcommand{\cC}[0]{\mathcal{C}}
\newcommand{\sD}[0]{\mathscr{D}}
\newcommand{\mD}[0]{\mathfrak D}
\newcommand{\cE}[0]{\mathcal{E}}%deprecated
\newcommand{\sE}[0]{\mathscr{E}}
\newcommand{\E}[0]{\mathbb{E}}
\newcommand{\EE}[0]{\mathop{\mathbb E}}
%\scalebox{1.25}{$\mathbb E$}}
\newcommand{\F}[0]{\mathbb{F}}
\newcommand{\cF}[0]{\mathcal{F}}
\newcommand{\sF}[0]{\mathscr{F}}
\newcommand{\G}[0]{\mathbb{G}}
\newcommand{\cG}[0]{\mathscr{G}}%deprecated.
\newcommand{\sG}[0]{\mathscr{G}}
\newcommand{\cH}[0]{\mathscr H}%deprecated
\newcommand{\sH}[0]{\mathscr H}
\newcommand{\Hq}[0]{\mathbb{H}}
\newcommand{\bfI}[0]{\mathbf{I}}
\newcommand{\I}[0]{\mathbb{I}}
\newcommand{\cI}[0]{\mathscr{I}}%deprecated
\newcommand{\sI}[0]{\mathscr{I}}
\newcommand{\cJ}[0]{\mathscr{J}}
\newcommand{\cK}[0]{\mathcal{K}}
\newcommand{\cL}[0]{\mathcal{L}}
\newcommand{\sL}[0]{\mathscr{L}}
\newcommand{\mM}[0]{\mathfrak{M}}
\newcommand{\N}[0]{\mathbb{N}}
\newcommand{\fN}[0]{\mathfrak{N}}
\newcommand{\cP}[0]{\mathcal{P}}
\newcommand{\Pj}[0]{\mathbb{P}}
\newcommand{\mP}[0]{\mathfrak{P}}
\newcommand{\mQ}[0]{\mathfrak{Q}}
%!
\newcommand{\cO}[0]{\mathcal{O}}
\newcommand{\sO}[0]{\mathscr{O}}
\newcommand{\Q}[0]{\mathbb{Q}}
\newcommand{\R}[0]{\mathbb{R}}
\newcommand{\bS}[0]{\mathbb{S}}
\newcommand{\T}[0]{\mathbb{T}}
\newcommand{\X}[0]{\mathfrak{X}}
\newcommand{\Z}[0]{\mathbb{Z}}
\newcommand{\one}[0]{\mathbbm{1}}
%lowercase
\newcommand{\mba}[0]{\mathbf{a}}%idele a
\newcommand{\ma}[0]{\mathfrak{a}}%ideal a
\newcommand{\mb}[0]{\mathfrak{b}}
\newcommand{\mc}[0]{\mathfrak{c}}
\newcommand{\mfd}[0]{\mathfrak d}
\newcommand{\mf}[0]{\mathfrak{f}}
\newcommand{\fg}[0]{\mathfrak{g}}
\newcommand{\vi}[0]{\mathbf{i}}%vector i
\newcommand{\vj}[0]{\mathbf{j}}
\newcommand{\vk}[0]{\mathbf{k}}
\newcommand{\mm}[0]{\mathfrak{m}}%ideal m
\newcommand{\mfp}[0]{\mathfrak{p}}
\newcommand{\mq}[0]{\mathfrak{q}}
\newcommand{\mr}[0]{\mathfrak{r}}
\newcommand{\mv}[0]{\mathbf{v}}
\newcommand{\mx}[0]{\mathbf{x}}%idele x
\newcommand{\my}[0]{\mathbf{y}}
%More sequences of letters
\newcommand{\et}[0]{_{\text{\'et}}}
\newcommand{\Gm}[0]{\mathbb{G}_m}
\newcommand{\Fp}[0]{\mathbb{F}_p}
\newcommand{\fq}[0]{\mathbb{F}_q}
\newcommand{\fpb}[0]{\ol{\mathbb{F}_p}}
\newcommand{\fpt}[0]{\mathbb{F}_p^{\times}}
\newcommand{\fqt}[0]{\mathbb{F}_q^{\times}}
\newcommand{\Kt}[0]{K^{\times}}
\newcommand{\RP}[0]{\mathbb{R}P}
\newcommand{\qb}[0]{\ol{\mathbb{Q}}}
\newcommand{\qp}[0]{\mathbb{Q}_p}
\newcommand{\qpb}[0]{\ol{\mathbb{Q}_p}}
\newcommand{\ql}[0]{\mathbb Q_{\ell}}
\newcommand{\sll}[0]{\mathfrak{sl}}
\newcommand{\vl}[0]{V_{\ell}}
\newcommand{\zl}[0]{\mathbb Z_{\ell}}
\newcommand{\zp}[0]{\mathbb Z_{p}}
\newcommand{\zpz}[0]{\mathbb Z/p\mathbb Z}
%Shortcuts for greek letters
\newcommand{\al}[0]{\alpha}
\newcommand{\be}[0]{\beta}
\newcommand{\ga}[0]{\gamma}
\newcommand{\Ga}[0]{\Gamma}
\newcommand{\de}[0]{\delta}
\newcommand{\De}[0]{\Delta}
\newcommand{\ep}[0]{\varepsilon}
\newcommand{\eph}[0]{\frac{\varepsilon}{2}}
\newcommand{\ept}[0]{\frac{\varepsilon}{3}}
\newcommand{\ka}[0]{\kappa}
\newcommand{\la}[0]{\lambda}
\newcommand{\La}[0]{\Lambda}
\newcommand{\ph}[0]{\varphi}
\newcommand{\Ph}[0]{\Phi}
\newcommand{\rh}[0]{\rho}
\newcommand{\te}[0]{\theta}
\newcommand{\Te}[0]{\Theta}
\newcommand{\vte}[0]{\vartheta}
\newcommand{\om}[0]{\omega}
\newcommand{\Om}[0]{\Omega}
\newcommand{\si}[0]{\sigma}
\newcommand{\Si}[0]{\Sigma}
\newcommand{\ze}[0]{\zeta}

%SYMBOLS

%Shortcuts for symbols
\newcommand{\nin}[0]{\not\in}
\newcommand{\opl}[0]{\oplus}
\newcommand{\bigopl}[0]{\bigoplus}
\newcommand{\ot}[0]{\otimes}
\newcommand{\bigot}[0]{\bigotimes}
\newcommand{\sub}[0]{\subset}
\newcommand{\nsub}[0]{\not\subset}
\newcommand{\subeq}[0]{\subseteq}
\newcommand{\supeq}[0]{\supseteq}
\newcommand{\nsubeq}[0]{\not\subseteq}
\newcommand{\nsupeq}[0]{\not\supseteq}
\newcommand{\nequiv}[0]{\not\equiv}
\newcommand{\bs}[0]{\backslash}
\newcommand{\iy}[0]{\infty}
\newcommand{\no}[0]{\trianglelefteq}%normal subgroup
\newcommand{\qeq}[0]{\stackrel?=}
\newcommand{\subsim}[0]{\stackrel{\sub}{\sim}}
\newcommand{\supsim}[0]{\stackrel{\supset}{\sim}}
\newcommand{\na}[0]{\nabla}
\newcommand{\mcv}[0]{*_-}
\newcommand{\dlim}[0]{\varinjlim}
\newcommand{\ilim}[0]{\varprojlim}
\newcommand{\gle}[0]{\begin{array}{c}
\ge\\
\le
\end{array}}
\newcommand{\lge}[0]{\begin{array}{c}
\le\\
\ge
\end{array}}
%\stackrel{-}{*}}%minus convoluion.

%COMMON TIME-SAVERS

%Fractions
\newcommand{\rc}[1]{\frac{1}{#1}}
\newcommand{\prc}[1]{\pa{\rc{#1}}}
\newcommand{\ff}[2]{\left\lfloor\frac{#1}{#2}\right\rfloor}
\newcommand{\cf}[2]{\left\lceil\frac{#1}{#2}\rceil\rfloor}
\newcommand{\fc}[2]{\frac{#1}{#2}}
\newcommand{\sfc}[2]{\sqrt{\frac{#1}{#2}}}
\newcommand{\pf}[2]{\pa{\frac{#1}{#2}}}%Shortcut for fraction with parentheses
\DeclareRobustCommand{\stl}{\genfrac\{\}{0pt}{}}

\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}%Partial derivatives
\newcommand{\dd}[2]{\frac{d #1}{d #2}}
\newcommand{\pdd}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ddd}[1]{\frac{d}{d #1}}
\newcommand{\af}[2]{\ab{\fc{#1}{#2}}}
\newcommand{\ddt}[2]{\frac{d^2 #1}{d {#2}^2}}
\newcommand{\pdt}[2]{\frac{\partial^2 #1}{\partial {#2}^2}}
\newcommand{\pdxy}[3]{\frac{\partial^2 #1}{\partial {#2}\partial {#3}}}
\newcommand{\pl}[0]{\partial}
\newcommand{\nb}[0]{\nabla}
\newcommand{\onb}[0]{\ol{\nabla}}
\newcommand{\dy}{\,dy}
\newcommand{\dx}{\,dx}

%Arrows
\newcommand{\lar}[0]{\leftarrow}
\newcommand{\ra}[0]{\rightarrow}
\newcommand{\dra}[0]{\dashrightarrow}
\newcommand{\lra}[0]{\leftrightarrow}
\newcommand{\rra}[0]{\twoheadrightarrow}
\newcommand{\hra}[0]{\hookrightarrow}
\newcommand{\tra}[0]{\twoheadrightarrow}
\newcommand{\send}[0]{\mapsto}
\newcommand{\xra}[1]{\xrightarrow{#1}}
\newcommand{\xla}[1]{\xleftarrow{#1}}
\newcommand{\xhra}[1]{\xhookrightarrow{#1}}
\newcommand{\xlra}[1]{\xleftrightarrow{#1}}
\newcommand{\xrc}[0]{\xrightarrow{\cong}}
\newcommand{\cir}[0]{\circlearrowright}
\newcommand{\cil}[0]{\circlearrowleft}

%Brackets
\newcommand{\ab}[1]{\left| {#1} \right|}
\newcommand{\an}[1]{\left\langle {#1}\right\rangle}
\newcommand{\ba}[1]{\left[ {#1} \right]}
\newcommand{\bc}[1]{\left\{ {#1} \right\}}
\newcommand{\bra}[1]{\langle{#1}|}
\newcommand{\braa}[1]{\langle\langle{#1}|}
\newcommand{\ce}[1]{\left\lceil {#1}\right\rceil}
\newcommand{\fl}[1]{\left\lfloor {#1}\right\rfloor}
\newcommand{\ro}[1]{\left\lfloor {#1}\right\rceil}
\newcommand{\ket}[1]{|{#1}\rangle}
\newcommand{\kett}[1]{|{#1}\rangle\rangle}
\newcommand{\bk}[2]{\langle{#1}|{#2}\rangle}
\newcommand{\braak}[2]{\langle\langle{#1}|{#2}\rangle\rangle}
\newcommand{\kbb}[1]{|{#1}\rangle\langle{#1}|}
\newcommand{\kb}[2]{|{#1}\rangle\langle{#2}|}
\newcommand{\kettb}[2]{|{#1}\rangle\rangle\langle\langle{#2}|}
\newcommand{\pa}[1]{\left( {#1} \right)}
\newcommand{\pat}[1]{\left( \text{#1} \right)}
\newcommand{\ve}[1]{\left\Vert {#1}\right\Vert}
\newcommand{\nv}[1]{\frac{#1}{\left\Vert {#1}\right\Vert}}
\newcommand{\nvl}[2]{\frac{#1}{\left\Vert {#1}\right\Vert_{#2}}}
\newcommand{\vvt}[1]{{#1}{#1}^\top}
\newcommand{\pvvt}[1]{\pa{#1}\pa{#1}^\top}
\newcommand{\vtv}[1]{{#1}^\top{#1}}
\newcommand{\pvtv}[1]{\pa{#1}^\top\pa{#1}}
\newcommand{\rb}[1]{\left.{#1}\right|}
\renewcommand{\nl}[1]{\left\Vert #1 \right\Vert_{L^1}}
\newcommand{\ad}[0]{|\cdot|}
\newcommand{\ved}[0]{\ve{\cdot}}
\renewcommand{\set}[2]{\left\{{#1}:{#2}\right\}}
\newcommand{\sett}[2]{\left\{\left.{#1}\right|{#2}\right\}}

%under and overlines, etc.
\newcommand{\ch}[1]{\check{#1}}
\newcommand{\dch}[1]{\check{\check{#1}}}
\newcommand{\olra}[1]{\overleftrightarrow{#1}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\ul}[1]{\underline{#1}}
\newcommand{\ub}[2]{\underbrace{#1}_{#2}}
\newcommand{\ora}[1]{\overrightarrow{#1}}
\newcommand{\ura}[1]{\underrightarrow{#1}}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\wh}[1]{\widehat{#1}}

%other
\newcommand{\fp}[1]{^{\underline{#1}}}%Falling power
\newcommand{\rp}[1]{^{\overline{#1}}}
\newcommand{\pp}[1]{^{(#1)}}
\newcommand{\sh}[0]{^{\sharp}}
\newcommand{\ri}[0]{\ddagger}%replace this with rosati involution
\newcommand{\bit}[0]{\{0,1\}}

%TEXT
\newcommand{\btih}[1]{\text{ by the induction hypothesis{#1}}}
\newcommand{\bwoc}[0]{by way of contradiction}
\newcommand{\by}[1]{\text{by~(\ref{#1})}}
\newcommand{\idk}[0]{{\color{red}I don't know.} }
\newcommand{\ore}[0]{\text{ or }}
\newcommand{\wog}[0]{ without loss of generality }
\newcommand{\Wog}[0]{ Without loss of generality }
\newcommand{\step}[1]{\noindent{\underline{Step {#1}:}}}
\newcommand{\prt}[1]{\noindent{\underline{Part {#1}:}}}
\newcommand{\tfae}[0]{ the following are equivalent}
\newcommand{\fabfm}[0]{for all but finitely many }

%FUNCTIONS
%Functions, etc.
\newcommand{\Abs}{(\text{Ab}/S)}
\newcommand{\abk}{(\text{Ab}/k)}
\newcommand{\abc}{(\text{Ab}/\C)}
\newcommand{\Alb}{\operatorname{Alb}}
\newcommand{\Ann}{\operatorname{Ann}}
\newcommand{\Area}{\operatorname{Area}}
\newcommand{\amax}{\operatorname{argmax}}
\newcommand{\amin}{\operatorname{argmin}}
\newcommand{\Ass}{\operatorname{Ass}}
\newcommand{\Art}{\operatorname{Art}}
\newcommand{\Aut}{\operatorname{Aut}}
\newcommand{\avg}{\operatorname{avg}}
\newcommand{\bias}[0]{\operatorname{bias}}
\newcommand{\Bin}{\operatorname{Bin}}
\newcommand{\Binom}{\operatorname{Binom}}
\newcommand{\Bl}[0]{\operatorname{Bl}}
\newcommand{\Br}{\operatorname{Br}}
\newcommand{\chr}{\operatorname{char}}
\newcommand{\cis}{\operatorname{cis}}
\newcommand{\cl}{\operatorname{Cl}}
%\newcommand{\Cl}{C}%changed notation%this is confusing
\newcommand{\Cl}{\operatorname{Cl}}
\newcommand{\Coh}{\operatorname{Coh}}
\newcommand{\Coinf}[0]{\operatorname{Coinf}}
\newcommand{\Coind}[0]{\operatorname{Coind}}
\newcommand{\coker}{\operatorname{coker}}
\newcommand{\colim}{\operatorname{colim}}
\newcommand{\Comp}{\operatorname{Comp}}
\newcommand{\conv}{\operatorname{conv}}
\newcommand{\oconv}{\ol{\conv}}
\newcommand{\Cor}{\operatorname{Cor}}
\newcommand{\Cov}{\operatorname{Cov}}
\newcommand{\cro}{\operatorname{cr}}
\newcommand{\degs}[0]{\deg_{\text{s}}}%separable degree
\newcommand{\Dec}{\operatorname{Dec}}
\newcommand{\depth}{\operatorname{depth}}
\newcommand{\Der}{\operatorname{Der}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\diam}{\operatorname{diam}}
\renewcommand{\div}{\operatorname{div}}
\newcommand{\Dir}{\operatorname{Dir}}
\newcommand{\Div}{\operatorname{Div}}
\newcommand{\Disc}{\operatorname{Disc}}%discrepancy
\newcommand{\disc}{\operatorname{disc}}%discriminant
\newcommand{\dom}{\operatorname{dom}}
\newcommand{\Ell}{\mathcal{E}{\rm{ll}}}
\newcommand{\Enc}{\operatorname{Enc}}
\newcommand{\End}{\operatorname{End}}
\newcommand{\Ent}{\operatorname{Ent}}
\newcommand{\Ext}{\operatorname{Ext}}
\newcommand{\Exp}{\operatorname{Exp}}
\newcommand{\err}{\operatorname{err}}
\newcommand{\ess}{\operatorname{ess}}
\newcommand{\ext}{\operatorname{ext}}
\newcommand{\pfcg}{(p\text{-FCGp}/k)}
\newcommand{\fcg}{(\text{FCGp}/k)}
\newcommand{\Frac}{\operatorname{Frac}}
\newcommand{\Frob}{\operatorname{Frob}}
\newcommand{\Fun}{\operatorname{Fun}}
\newcommand{\FS}{\operatorname{FS}}
\newcommand{\Gal}{\operatorname{Gal}}
\newcommand{\Gap}{\operatorname{Gap}}
\newcommand{\grad}{\operatorname{grad}}
\newcommand{\GL}{\operatorname{GL}}
\newcommand{\gps}{(\text{Gp}/S)}
\newcommand{\Hess}{\operatorname{Hess}}
\newcommand{\Het}{H_{\text{\'et}}}
\newcommand{\Hom}{\operatorname{Hom}}
\newcommand{\Homeo}{\operatorname{Homeo}}
\newcommand{\chom}[0]{\mathscr{H}om}
\newcommand{\Homc}{\operatorname{Hom}_{\text{cont}}}
\newcommand{\id}{\mathrm{id}}
\newcommand{\Id}{\operatorname{Id}}
\newcommand{\im}[0]{\text{im}}
\newcommand{\imp}[0]{\im^{\text{pre}}}
\newcommand{\Ind}[0]{\operatorname{Ind}}
\newcommand{\Inf}[0]{\operatorname{Inf}}
\newcommand{\inv}[0]{\operatorname{inv}}
\newcommand{\Isoc}[0]{\operatorname{Isoc}}
\newcommand{\Isog}[0]{\operatorname{Isog}}
\newcommand{\Isom}[0]{\operatorname{Isom}}
\newcommand{\KL}[0]{\operatorname{KL}}
\newcommand{\Jac}[0]{\operatorname{Jac}}
\newcommand{\li}[0]{\operatorname{li}}
\newcommand{\Li}[0]{\operatorname{li}}
\newcommand{\Lie}[0]{\operatorname{Lie}}
\newcommand{\Line}[0]{\operatorname{Line}}
\newcommand{\Lip}[0]{\operatorname{Lip}}
\newcommand{\lcm}[0]{\operatorname{lcm}}
\newcommand{\Mat}{\operatorname{Mat}}
\newcommand{\Mod}{\operatorname{Mod}}
\newcommand{\Dmod}{\Mod_{W[F,V]}^{\text{fl}}}
\newcommand{\nil}[0]{\operatorname{nil}}
\newcommand{\nm}{\operatorname{Nm}}
\newcommand{\NS}{\operatorname{NS}}
\newcommand{\ord}{\operatorname{ord}}
\newcommand{\osc}{\operatorname{osc}}
\newcommand{\PDer}{\operatorname{PDer}}
\newcommand{\PGL}{\operatorname{PGL}}
\newcommand{\Pic}{\operatorname{Pic}}
\newcommand{\Pico}{\operatorname{Pic}^{\circ}}
\newcommand{\Pois}{\operatorname{Pois}}
\newcommand{\poly}{\operatorname{poly}}
\newcommand{\polylog}{\operatorname{polylog}}
\newcommand{\PSL}{\operatorname{PSL}}
\newcommand{\Per}{\operatorname{Per}}
\newcommand{\perm}{\operatorname{perm}}
\newcommand{\PrePer}{\operatorname{PrePer}}
\newcommand{\Prob}{\operatorname{Prob}}
\newcommand{\Proj}{\operatorname{Proj}}
\newcommand{\Prj}[0]{\textbf{Proj}}
\newcommand{\QCoh}{\operatorname{QCoh}}
\newcommand{\Rad}{\operatorname{Rad}}
\newcommand{\range}{\operatorname{range}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\red}{\operatorname{red}}
\newcommand{\Reg}{\operatorname{Reg}}
\newcommand{\Res}{\operatorname{Res}}
\newcommand{\Ric}{\operatorname{Ric}} %Ricci curvature
\newcommand{\rot}{\operatorname{rot}}
\newcommand{\Scal}{\operatorname{Scal}} %Ricci curvature
\newcommand{\schs}{(\text{Sch}/S)}
\newcommand{\schk}{(\text{Sch}/k)}
\newcommand{\se}{\text{se}}
\newcommand{\srank}{\text{srank}}
\newcommand{\hse}{\wh{\text{se}}}
\newcommand{\Sel}{\operatorname{Sel}}
\newcommand{\sens}{\operatorname{sens}}
\newcommand{\Set}{(\text{Set})}
\newcommand{\sgn}{\operatorname{sign}}
\newcommand{\sign}{\operatorname{sign}}
\newcommand{\SL}{\operatorname{SL}}
\newcommand{\SO}{\operatorname{SO}}
\newcommand{\Spec}{\operatorname{Spec}}
\newcommand{\Specf}[2]{\Spec\pa{\frac{k[{#1}]}{#2}}}
\newcommand{\rspec}{\ul{\operatorname{Spec}}}
\newcommand{\Spl}{\operatorname{Spl}}
\newcommand{\spp}{\operatorname{sp}}
\newcommand{\spn}{\operatorname{span}}
\newcommand{\Stab}{\operatorname{Stab}}
\newcommand{\SU}{\operatorname{SU}}
\newcommand{\Supp}{\operatorname{Supp}}
\newcommand{\ssupp}{\operatorname{sing}\operatorname{supp}}
\newcommand{\Sym}{\operatorname{Sym}}
\newcommand{\Th}{\operatorname{Th}}
\newcommand{\Tor}{\operatorname{Tor}}
\newcommand{\tor}{\operatorname{tor}}
\newcommand{\Tr}[0]{\operatorname{Tr}}
\newcommand{\tr}[0]{\operatorname{tr}}
\newcommand{\TV}[0]{\textup{TV}}
\newcommand{\val}[0]{\text{val}}
\newcommand{\Var}[0]{\operatorname{Var}}
\newcommand{\var}[0]{\text{var}}
\newcommand{\vcong}{\operatorname{vcong}}
\newcommand{\Vol}[0]{\text{Vol}}
\newcommand{\vol}[0]{\text{vol}}
\providecommand{\cal}[1]{\mathcal{#1}}
\renewcommand{\cal}[1]{\mathcal{#1}}
\providecommand{\bb}[1]{\mathbb{#1}}
\renewcommand{\bb}[1]{\mathbb{#1}}

%Text super/subscripts
\newcommand{\abe}[0]{^{\text{ab}}}
\newcommand{\gal}[0]{^{\text{gal}}}%galois closure
%\newcommand{\op}{^{\text{op}}}
\newcommand{\pre}[0]{^{\text{pre}}}
\newcommand{\rd}[0]{_{\text{red}}}
\newcommand{\sep}[0]{^{\text{sep}}}
\newcommand{\tp}{^{\text{top}}}
\newcommand{\tors}{_{\text{tors}}}
\newcommand{\ur}[0]{^{\text{ur}}}
\newcommand{\urt}[0]{^{\text{ur}\times}}

%COMMUTATIVE DIAGRAMS

%Commutative diagram shortcuts
\newcommand{\commsq}[8]{\xymatrix{#1\ar[r]^-{#6}\ar[d]_{#5} &#2\ar[d]^{#7} \\ #3 \ar[r]^-{#8} & #4}}
%Makes a diagram like this
%1->2
%|    |
%3->4
%Arguments 5, 6, 7, 8 on arrows
%  6
%5  7
%  8
\newcommand{\pull}[9]{
#1\ar@/_/[ddr]_{#2} \ar@{.>}[rd]^{#3} \ar@/^/[rrd]^{#4} & &\\
& #5\ar[r]^{#6}\ar[d]^{#8} &#7\ar[d]^{#9} \\}
\newcommand{\back}[3]{& #1 \ar[r]^{#2} & #3}
%Syntax:\pull 123456789 \back ABC
%1=upper left-hand corner
%2,3,4=arrows from upper LH corner, going down, diagonal, right
%5,6,7=top row (6 on arrow)
%8,9=middle rows (on arrows)
%A,B,C=bottom row
%composition
\newcommand{\cmp}[9]{
\xymatrix{
#1 \ar[r]^{#4}{#5} \ar@/_2pc/[rr]^{#8}_{#9} & #2 \ar[r]^{#6}_{#7} & #3
}
}
\newcommand{\ctr}[9]{
\xymatrix{
#1 \ar[rr]^{#4}_{#5}\ar[rd]^{#6}_{#7} && #2\ar[ld]_{#8}^{#9}\\
& #3 &
}
}
\newcommand{\ctrr}[9]{
\xymatrix{
#1 \ar[rr]^{#4}_{#5} && #2\\
& #3 \ar[lu]_{#6}^{#7}\ar[ru]_{#8}^{#9}&
}
}

\newcommand{\ctri}[9]{
\xymatrix{
#1 \ar[rr]^{#4}_{#5}\ar[rd]^{#6}_{#7} && #2\\
& #3 \ar[ru]^{#8}_{#9}&
}
}
\newcommand{\rcommsq}[8]{\xymatrix{#1 &#2\ar[l]_-{#6} \\ #3 \ar[u]^{#5} & #4 \ar[u]_{#7}\ar[l]_-{#8}}}


%Arrow shortcuts
\newcommand{\ha}[1]{\ar@{^(->}[#1]}
\newcommand{\ls}[1]{\ar@{-}[#1]}
\newcommand{\sj}[1]{\ar@{->>}[#1]}
\newcommand{\aq}[1]{\ar@{=}[#1]}
\newcommand{\acir}[1]{\ar@{}[#1]|-{\textstyle{\circlearrowright}}}
\newcommand{\acil}[1]{\ar@{}[#1]|-{\textstyle{\circlearrowleft}}}
\newcommand{\ard}[1]{\ar@{.>}[#1]}
\newcommand{\mt}[1]{\ar@{|->}[#1]}
\newcommand{\inm}[1]{\ar@{}[#1]|-{\in}}
\newcommand{\inr}{\ar@{}[d]|-{\rotatebox[origin=c]{-90}{$\in$}}}
\newcommand{\inl}{\ar@{}[u]|-{\rotatebox[origin=c]{90}{$\in$}}}

%Other
%\newcommand{\set}[2]{\left.\left\{{#1}\right|{#2}\right\}}
%\newcommand{\sett}[2]{\left\{{#1}\left|{#2}\right\}\right.}

%SUMS, ETC.
\newcommand{\sumr}[2]{\sum_{\scriptsize \begin{array}{c}{#1}\\{#2}\end{array}}}%sum with 2 rows
\newcommand{\prr}[2]{\prod_{\scriptsize \begin{array}{c}{#1}\\{#2}\end{array}}}%product with 2 rows
\newcommand{\maxr}[2]{\max_{\scriptsize \begin{array}{c}{#1}\\{#2}\end{array}}}%product with 2 rows
\newcommand{\minr}[2]{\min_{\scriptsize \begin{array}{c}{#1}\\{#2}\end{array}}}%product with 2 rows
\newcommand{\trow}[2]{\scriptsize \begin{array}{c}{#1}\\{#2}\end{array}}
\newcommand{\seqo}[3]{\{#3\}_{#1=1}^{#2}}
\newcommand{\seqos}[3]{\{#3_#1\}_{#1=1}^{#2}}
\newcommand{\seqz}[3]{\{#3\}_{#1=0}^{#2}}
\newcommand{\seqzs}[3]{\{#3_#1\}_{#1=0}^{#2}}
\newcommand{\su}[0]{\sum_{n=0}^{\iy}}
\newcommand{\suo}[0]{\sum_{n=1}^{\iy}}
\newcommand{\sumo}[2]{\sum_{#1=1}^{#2}}
\newcommand{\sumz}[2]{\sum_{#1=0}^{#2}}
\newcommand{\prodo}[2]{\prod_{#1=1}^{#2}}
\newcommand{\prodz}[2]{\prod_{#1=0}^{#2}}
\newcommand{\oplo}[2]{\bigopl_{#1=1}^{#2}}
\newcommand{\cupo}[2]{\bigcup_{#1=1}^{#2}}
\newcommand{\capo}[2]{\bigcap_{#1=1}^{#2}}
\newcommand{\iiy}[0]{\int_0^{\infty}}
\newcommand{\iny}[0]{\int_{-\infty}^{\infty}}
\newcommand{\iiiy}[0]{\int_{-\infty}^{\infty}}%DEPRECATED
\newcommand{\sui}[0]{\sum_{i=1}^{n}}
\newcommand{\suiy}[0]{\sum_{i=1}^{\iy}}
\newcommand{\cui}[0]{\bigcup_{i=1}^n}
\newcommand{\suj}[0]{\sum_{j=1}^{n}}
\newcommand{\suij}[0]{\sum_{i,j}}
\newcommand{\limn}[0]{\lim_{n\to \infty}}

%MATRICES

%Matrices
\newcommand{\scoltwo}[2]{
\left(\begin{smallmatrix}
{#1}\\
{#2}
\end{smallmatrix}\right)}
\newcommand{\coltwo}[2]{
\begin{pmatrix}
{#1}\\
{#2}
\end{pmatrix}}
\newcommand{\colthree}[3]{
\begin{pmatrix}
{#1}\\
{#2}\\
{#3}
\end{pmatrix}
}
\newcommand{\colfour}[4]{
\begin{pmatrix}
{#1}\\
{#2}\\
{#3}\\
{#4}
\end{pmatrix}
}
\newcommand{\cth}[3]{
\begin{pmatrix}
{#1}\\
{#2}\\
{#3}
\end{pmatrix}
}
\newcommand{\detm}[4]{
\ab{
\begin{matrix}
{#1}&{#2}\\
{#3}&{#4}
\end{matrix}
}}
\newcommand{\sdetm}[4]{
\ab{
\begin{smallmatrix}
{#1}&{#2}\\
{#3}&{#4}
\end{smallmatrix}
}}
\newcommand{\matt}[4]{
\begin{pmatrix}
{#1}&{#2}\\
{#3}&{#4}
\end{pmatrix}
}
\newcommand{\smatt}[4]{
\left(\begin{smallmatrix} 
{#1}&{#2}\\
{#3}&{#4}
\end{smallmatrix}\right)
}
\newcommand{\mattn}[9]{
\begin{pmatrix}
{#1}&{#2}&{#3}\\
{#4}&{#5}&{#6}\\
{#7}&{#8}&{#9}
\end{pmatrix}
}

\newcommand{\bt}[2]{
\left\{\begin{matrix}
\text{#1}\\
\text{#2}
\end{matrix}
\right\}}
\newcommand{\bth}[3]{
\left\{\begin{matrix}
\text{#1}\\
\text{#2}\\
\text{#3}
\end{matrix}
\right\}}

\newcommand{\tcase}[4]{
\begin{cases}
#1 & #2\\
#3 & #4
\end{cases}}
\newcommand{\txcase}[4]{
\begin{cases}
#1 & \text{#2}\\
#3 & \text{#4}
\end{cases}}

\newcommand{\ifoth}[3]{
\begin{cases}
#1 & \text{if }#2\\
#3 & \text{otherwise}
\end{cases}}

%EQUATIONS
\newcommand{\beq}[1]{\begin{equation}\llabel{#1}}
\newcommand{\eeq}[0]{\end{equation}}
\newcommand{\bal}[0]{\begin{align*}}
\newcommand{\eal}[0]{\end{align*}}%this doesn't work; i don't know why
\newcommand{\ban}[0]{\begin{align}}
\newcommand{\ean}[0]{\end{align}}
\newcommand{\ig}[2]{\begin{center}\includegraphics[scale=#2]{#1}\end{center}}
\newcommand{\ign}[2]{\includegraphics[scale=#2]{#1}}

%COURSE-SPECIFIC

%measure theory, analysis
\newcommand{\am}[0]{(a.e., $\mu$)}
\newcommand{\ftla}[1]{\int e^{i\lambda\cdot x}{#1}\,d\lambda}
\newcommand{\lime}[0]{\lim_{\varepsilon\to 0}}

%number theory
\newcommand{\modt}[1]{\,(\text{mod}^{\times}\, {#1})}
\newcommand{\tl}[0]{T_{\ell}}
 %multiplicative subgroup
\newcommand{\zmod}[1]{\Z/{#1}\Z}
\newcommand{\md}[1]{\,(\text{mod }#1)}
\newcommand{\ks}[1]{K(\sqrt{#1})}
\newcommand{\ksq}[1]{K(\sqrt{#1})/K}
\newcommand{\nksq}[1]{\nm_{K(\sqrt{#1})/K}(K(\sqrt{#1})^{\times})}
\newcommand{\mpp}[0]{\mP/\mfp}

%manifolds
\newcommand{\cvd}[0]{\frac{D}{\partial t}}
\newcommand{\cvs}[0]{\frac{D}{\partial s}}
\newcommand{\np}[1]{\nabla_{\pd{}{#1}}}

%algebraic geometry
\newcommand{\av}[0]{A^{\vee}}


%arithmetic combinatorics
\newcommand{\Deq}[1]{\Delta^{\times}_{#1}}

%modular forms
\newcommand{\GLAi}[0]{\text{GL}_2(\mathbb A)_{\infty}}

%noise sensitivity part iii essay
\newcommand{\Dict}[0]{\operatorname{\mathsf{Dict}}}
\newcommand{\Maj}[0]{\operatorname{\mathsf{Maj}}}
\newcommand{\MAJ}[0]{\operatorname{\mathsf{Maj}}}
\newcommand{\Parity}[0]{\operatorname{\mathsf{Parity}}}
\newcommand{\Tribes}[0]{\operatorname{\mathsf{Tribes}}}
\newcommand{\Ns}[0]{\operatorname{NS}}
\newcommand{\DT}[0]{\operatorname{\mathsf{DT}}}
\newcommand{\DNF}[0]{\operatorname{\mathsf{DNF}}}
\newcommand{\CNF}[0]{\operatorname{\mathsf{CNF}}}
\newcommand{\Circuit}[0]{\operatorname{\mathsf{Circuit}}}
\newcommand{\Ac}[0]{\mathsf{AC}}
\newcommand{\EB}[0]{\text{EB}}
%comp complexity
%complexity theory
\newcommand{\ACC}[0]{\operatorname{\mathsf{ACC}}}
\newcommand{\BPP}[0]{\mathsf{BPP}}
\newcommand{\BPTIME}[0]{\operatorname{\mathsf{BPTIME}}}
\newcommand{\CLIQUE}[0]{\operatorname{\mathsf{CLIQUE}}}
\newcommand{\EXP}[0]{\mathsf{EXP}}
\newcommand{\NEXP}[0]{\mathsf{NEXP}}
\newcommand{\NC}[0]{\operatorname{\mathsf{NC}}}
\newcommand{\NP}[0]{\operatorname{\mathsf{NP}}}
\newcommand{\NTIME}[0]{\operatorname{\mathsf{NTIME}}}
\newcommand{\msP}[0]{\operatorname{\mathsf{P}}}
\newcommand{\PCP}[0]{\operatorname{\mathsf{PCP}}}
\newcommand{\SAT}[0]{\mathsf{SAT}}
\newcommand{\SUBEXP}[0]{\mathsf{SUBEXP}}
\newcommand{\TIME}[0]{\operatorname{\mathsf{TIME}}}
\newcommand{\zz}{\textcircled{Z}}
%statistics
\newcommand{\hten}[0]{\widehat{\theta_n}}

%EDITING HELP
%blu: key idea or concept. red: unresolved issue/question. 
\newcommand{\blu}[1]{{\color{blue}#1}}
\newcommand{\grn}[1]{{\color{green}#1}}
\newcommand{\redd}[1]{{\color{red}#1}}
\newcommand{\pur}[1]{{\color{purple}#1}}
\newcommand{\oge}[1]{{\color{orange}#1}}
\newcommand{\concept}[1]{#1}
\newcommand{\fixme}[1]{{\color{red}#1}}
\newcommand{\cary}[1]{{\color{purple}#1}}%deprecated
%short for commentary
\newcommand{\llabel}[1]{\label{#1}\text{\fixme{\tiny#1}}}
\newcommand{\nref}[1]{\ref{#1}}
%%%%%%%%%%%
%Use the above when working on the document, so labels will be displayed by their theorems, and you can write reminders to yourself. Switch to the below commands when publishing.
%%%%%%%%%%%
%\newcommand{\fixme}[1]{}
%\newcommand{\concept}[1]{{\color{blue}#1}}
%\newcommand{\llabel}[1]{\label{#1}}
%%%%%%%%%%%

\newcommand{\itag}[1]{\index{#1}[\##1]}
\newcommand{\ilbl}[1]{[#1]\index{#1}}
\newcommand{\iadd}[1]{\index{#1} #1}
\newcommand{\arxiv}[1]{\url{http://www.arxiv.org/abs/#1}}

%markup
\newcommand{\ivocab}[1]{\index{#1}\textbf{#1}}
\newcommand{\vocab}[1]{\textbf{#1}} %also index automatically.
\newcommand{\summq}[1]{\textbf{Summary Question: }#1}
\newcommand{\keypt}[1]{{\it #1}}
\newcommand{\subprob}[1]{\noindent\textbf{#1}\\}
\newcommand{\qatable}[1]{\begin{center}
    \begin{longtable}{ | p{5.5cm} | p{10cm} |}
#1
\end{longtable}
\end{center}}

%Page breaks in equations
\allowdisplaybreaks[2]

%SHA
\DeclareFontFamily{U}{wncy}{}
    \DeclareFontShape{U}{wncy}{m}{n}{<->wncyr10}{}
    \DeclareSymbolFont{mcy}{U}{wncy}{m}{n}
    \DeclareMathSymbol{\Sh}{\mathord}{mcy}{"58} 

==> main.tex <==
% %\documentclass[11pt]{article}
% \documentclass[anon,12pt]{colt2022}
% \usepackage{times} % colt font

% \input{packages_colt}
% %\input{packages_arxiv.tex}
% \input{theorems_std.tex}
% \input{macros_colt.tex}

% %\usepackage{algorithm,algorithmicx,algpseudocode}

% %\usepackage{etoolbox}

% % \algrenewcommand\algorithmicrequire{\textbf{Input:}}
% % \algrenewcommand\algorithmicensure{\textbf{Output:}}

% % \algblockdefx{Block}{EndBlock}[1]{#1}[0]{}
% % \algtext*{EndBlock}
% % %\algblockdefx{Block}{EndBlock}[2][]{\textbf{#1} #2}[0]{}
% % %\algblockloopx{Block}{EndBlock}[1]{#1}[0]{}

% % % continuation indent patch http://tex.stackexchange.com/questions/78776/forced-indentation-in-algorithmicx
% % \newlength{\continueindent}
% % \setlength{\continueindent}{2em}
% % \usepackage{etoolbox}
% % \makeatletter
% % \newcommand*{\ALG@customparshape}{\parshape 2 \leftmargin \linewidth \dimexpr\ALG@tlm+\continueindent\relax \dimexpr\linewidth+\leftmargin-\ALG@tlm-\continueindent\relax}
% % \apptocmd{\ALG@beginblock}{\ALG@customparshape}{}{\errmessage{failed to patch}}
% % \makeatother
% % end continuation indent patch

% % FOR ARXIV/BIBLATEX version
% %\addbibresource{bib.bib}

% \newcommand{\sech}[0]{\operatorname{sech}}
% \newcommand{\prl}[0]{\parallel}

% \definecolor{purple}{rgb}{0.5, 0.0, 0.5}
% \newcommand{\hlnote}[1]{\textcolor{red}{\textbf{HL:} #1}}
% \newcommand{\fnote}[1]{\textcolor{purple}{\textbf{FK:} #1}}
% \newcommand{\anote}[1]{\textcolor{purple}{\textbf{AR:} #1}}


% \newcommand{\CP}[0]{C_{\textup{P}}}
% \newcommand{\CLS}[0]{C_{\textup{LS}}}
% \newcommand{\CMLS}[0]{C_{\textup{MLS}}}
% \newcommand{\bi}[0]{\mathbf i}

% \newcommand{\BC}[0]{\{\pm 1\}^n}
% \newcommand{\sBC}[0]{\sum_{\si\in \{\pm 1\}^n}}

% \newcommand{\Grid}[0]{\textup{Grid}_{L,\eta}^d}

% \newcommand{\ZJh}[0]{Z_{J,h}}
% \newcommand{\Zjoint}[0]{Z_{J,h}^{\textup{joint}}}
% \newcommand{\Zproj}[0]{Z_{J^\prl,J^\perp,h}}
% %{Z_{J,h,J^\prl}}
% \newcommand{\pproj}[0]{p_{J^\prl,J^\perp,h}}
% \newcommand{\Pproj}[0]{P_{J^\prl,J^\perp,h}}
% \newcommand{\isingexp}[2]{\rc 2 \an{\si, #1 \si} + \an{#2, \si}}
% \newcommand{\ising}[2]{\exp\pa{\isingexp{#1}{#2}}}
% \newcommand{\Jhs}[0]{\isingexp{J}{h}}
% \newcommand{\eJhs}[0]{\exp\pa{\isingexp{J}{h}}}
% \newcommand{\Jpall}[0]{J^\perp_{\textup{all}}}
% \newcommand{\Pst}[0]{P^{\textup{st}}}
% \newcommand{\pst}[0]{p^{\textup{st}}}
% \newcommand{\op}[0]{\textup{op}}

% \begin{document}


% %\title{Sampling and partition function estimation for approximately low-rank Ising models}
% \title{Sampling Approximately Low-Rank Ising Models: \\ MCMC meets Variational Methods}
% %\title{Sampling from Ising models with a few large eigenvalues}
% %Fred: maybe "spike eigenvalues" or "spectral outliers" would be more detailed and sound better than low rank
% %or "approximately low rank"?
% %Another option: something like "bounded spectral bulk"?

% \coltauthor{Frederic Koehler, \quad Holden Lee\thanks{Department of Mathematics,
% Duke University.
% %Email: \texttt{holden.lee@duke.edu}
% }, \quad Andrej Risteski}


% \date{\today}
% \maketitle
% \begin{abstract}
%     We consider Ising models on the hypercube with a general interaction matrix $J$, and give a polynomial time sampling algorithm when all but $O(1)$ eigenvalues of $J$ lie in an interval of length one, a situation which occurs in many models of interest. This was previously known for the Glauber dynamics when \emph{all} eigenvalues fit in an interval of length one; however, a single outlier can force the Glauber dynamics to mix torpidly. Our general result implies the first polynomial time sampling algorithms for low-rank Ising models such as Hopfield networks with a fixed number of patterns and Bayesian clustering models with low-dimensional contexts, 
%     and greatly improves the polynomial time sampling regime for the antiferromagnetic/ferromagnetic Ising model with inconsistent field on expander graphs. It also improves on previous approximation algorithm results based on the naive mean-field approximation in variational methods and statistical physics. 
    
%     Our approach is based on a new fusion of ideas from the MCMC and variational inference worlds. As part of our algorithm, we define a new nonconvex variational problem which allows us to sample from an exponential reweighting of a distribution by a negative definite quadratic form, and show how to make this procedure provably efficient using stochastic gradient descent. On top of this, we construct a new simulated tempering chain (on an extended state space arising from the Hubbard-Stratonovich transform) which overcomes the obstacle posed by large positive eigenvalues, and combine it with the SGD-based sampler to solve the full problem. 
% \end{abstract}

% %TODO:
% %\begin{enumerate}
% %    \item Add introduction.
% %    \item \hlnote{Add more details to sampling section.}
% %    \item Import the negative definite writeup.
% %    \item Show how to do partition function estimation and sampling with negative definite components.
% %    \item Add examples/applications. \fnote{mostly done, clean up appendix.}% \fnote{two applications to classic models: SK Model with Ferromagnetic Interaction \cite{chen2014mixed,talagrand2010mean}. Hopfield model with a fixed number of patterns \cite{gentz1999fluctuations,talagrand2010mean}.} \fnote{add antiferromagnetic/max-cut ising model on random $d$-regular graph} \fnote{clean up GMM and Contextual SBM example}
%     %Q: can you do importance sampling with original convex relaxation?
% %    \item \fnote{remember to add comparison to $\|J\|_F^2$ condition from variational inference results somewhere (by considering the interval $[-1/2,1/2]$ as the bulk, we should reproduce similar results but now sampling?)}
    
% %    \fnote{pick one of $x$ and $\sigma$ to denote spin} \hlnote{Let's use $\si$ because I used $x_i$ to denote columns of $X$} %fixed
% %\end{enumerate}

% %Refs: \cite{eldan2020spectral,anari2021aentropic}, \cite{jain2019mean}



% \input{intro}
% \input{overview}

% %\input{old-alg}

% \section{Applications}\label{sec:applications}
% Our results specialize to give new sampling guarantees for a many models of interest.  All of these are Ising models, so in each application we will describe the particular interaction matrix which arises and the resulting runtime guarantee. In all of the applications, the behavior in the presence of an external field $h \in \mathbb{R}^n$ is of interest (for example, in the Hopfield network to preferentially weight the distribution towards a particular memory) and %our results automatically apply to 
% we automatically handle this case. 

% \paragraph{Hopfield Network with a fixed number of patterns.} The Hopfield network is a neural model of associative memory 
% %driven by a Hebbian learning rule 
% (\cite{hopfield1982neural}, see also \cite{pastur1977exactly,pastur1978theory,little1974existence}) which has been hugely influential and extensively studied. In particular, for rigorous mathematical results see the textbooks by \cite{bovier2012mathematical,talagrand2010mean}.
% Formally, given patterns $\eta_1,\ldots,\eta_m \in \{\pm 1\}^n$ the Hopfield network at inverse temperature $\beta$ is the Ising model with interaction matrix
% $J = \frac{\beta}{2n} \sum_{v = 1}^m \eta_v \eta_v^\top$.
% This is thought of as a ``Hebbian'' learning rule because for each memory $\eta_v$ and neurons (coordinates) $i$ and $j$, the term $(\eta_v)_i (\eta_v)_j$ is positive if $(\eta_v)_i = (\eta_v)_j$ and negative otherwise. Therefore if $J$ is thought of as the ``wiring'' of the neurons, then for each pattern all of the neurons which ``fire together," i.e., have the same spin, are ``wired together''.
% %, matching the idiom that ``neurons which fire together wire together''. 

% Most of the interest in this model has been in the case of low/zero-temperature, which means the parameter $\beta$ is large. 
% Glauber dynamics (Gibbs sampling) has long been considered as a natural dynamics for the Hopfield network. Informally, the patterns stored in the network serve as ``attractors'' which trap the dynamics. This is interesting as %it can be thought of as a 
% in a sense it means the network exhibits memory; however, from the sampling perspective this means that the vanilla Glauber dynamics are not expected to mix in the most interesting regime of this model.

% When the number of patterns $m$ is fixed (a regime which has been rigorously studied in e.g., \cite{gentz1999fluctuations,bovier2012mathematical,talagrand2010mean}), we obtain the first polynomial time sampling algorithm for the Gibbs measure of this model that works for any fixed $\beta > 0$. Based on the rigorous results in this model (see \cite{bovier2012mathematical,talagrand2010mean}), when each pattern is independently sampled $\eta_i \sim \mathsf{Uniform} (\{\pm 1\}^n)$ and $\beta > 1$ the distribution will be almost entirely supported on $2m$ clusters corresponding to each of the patterns $\{\pm \eta_i\}_{i = 1}^m$ and so ordinary Glauber dynamics will not mix rapidly. (This should not be too difficult to formally prove given their results, though we did not do this.) Note that our sampling results apply to arbitrary patterns $\eta_i$, not just the commonly studied case where the patterns are uniformly random from the hypercube. 


% \paragraph{Antiferromagnetic and Ferromagnetic Ising Model on expanders and random graphs.} Suppose that $A$ is the adjacency matrix of a graph; then the \emph{antiferromagnetic Ising model} at inverse temperature $\beta$ has interaction matrix
% $J = -\beta A$.
% It is known that for worst-case graphs of maximum degree $d$, that polynomial time sampling is only possible for $\beta = O(1/d)$ (\cite{sly2012computational}, in fact the precise threshold is known as a function of $d$). However, this should be far from tight in other cases of interest, such as on a uniformly random $d$-regular graph: in this model, it is known that the symmetry breaking phase transition is at scaling $\beta = \Theta(1/\sqrt{d})$ (see \cite{coja2020ising} and references within) and we would expect the sampling regime of the model to be similar. 
% %when $A$ is a spectral expander and we can prove it as a consequence of our main result. 

% Based on our main result, we can indeed recover the correct scaling in the random $d$-regular graph setting, as a special case of a much more generic result about spectral expanders.
% Let $\lambda = \max\{|\lambda_2(A)|, |\lambda_n(A)|\}$; then our results give a polynomial time sampler whenever $\beta d = O(\log n)$ (so that our algorithm is polynomial time) %\hlnote{Do you mean $\be d$ here?} %fixed
% and provided
% $\beta \lambda < 1$.
% For example, in the case of a \emph{Ramanujan graph} of degree $d$ we have $\lambda \le 2\sqrt{d - 1}$ and so we can sample in polynomial time whenever
% $\beta < \frac{1}{2\sqrt{d - 1}}$,
% which is a dramatic improvement over $O(1/d)$. Because of Friedman's Theorem, we know the same result holds for the a uniformly random $d$-regular graph since it will be almost-Ramanujan \citep{friedman2008proof}. Note that it is the presence of the ``trivial'' eigenvalue $\lambda_1$ which prevents the result from being deduced from the pre-existing works (e.g., \cite{eldan2020spectral}) which can handle related models (diluted $d$-regular SK model) without outlier eigenvalues.  Our result also applies analogously if there are a couple of outlier eigenvalues, e.g., on bipartite expanders.  

% A completely analogous consequence of our theory is for the case of \emph{ferromagnetic} Ising models on expanders, where we have $J = \beta A$. In this case, the famous result of Jerrum and Sinclair \citep{jerrum1993polynomial} proves that sampling is possible when the external field $h$ is \emph{consistent} i.e., $h_i \ge 0$ for all $i$. However, when the signs of the external fields $h_i$ are allowed to disagree, sampling from the ferromagnetic Ising model is \#BIS-Hard \citep{goldberg2007complexity}. So our result also implies sampling algorithms for the ferromagnetic Ising model with inconsistent external field on expanders up to larger inverse temperatures than were previously known. 

% %Finally, in the case of bipartite expanders (with either ferromagnetic or antiferromagnetic, $A$ will have both a single large positive and a single large negative eigenvalue. Again, our sampling algorithm allows for sampling 
% %\paragraph{Ferromagnetic Ising Model on expanders and with inconsistent fields.} TODO: emphasize that Jerrum-Sinclair does not apply when external fields are inconsistent, but our result does. 

% %\paragraph{Ising model on bipartite expanders.} This application gives an intuitive example where both a positive and a negative spike eigenvalues are present.  

% \paragraph{Sherrington-Kirkpatrick Model with Ferromagnetic Interaction.} The Sherrington-Kirkpatrick model is one of the most famous spin glass models, and the SK model with ferromagnetic interactions is a natural variant which exhibits a combination of ferromagnetic and spin glass behaviors---see e.g., \cite{chen2014mixed,comets1999sherrington,talagrand2010mean} for rigorous probabilistic analysis of this model. The interaction matrix $J$ is given by
% $J_{ij} = \frac{\beta_1}{n}  + \beta_2 W_{ij}$
% where $W$ is a matrix sampled from the Gaussian Orthogonal Ensemble (so $W_{ij} \sim N(0,1/n)$). Since $\|W\|_{\op} \le 2(1 + o(1))$ with high probability by classical results in random matrix theory \citep{anderson2010introduction}, we are able to sample in polynomial time from this model for any fixed $\beta_1$, as long as $\beta_2 < 1/4$. 


% \paragraph{Posterior in Low-Dimensional Gaussian Mixture Model.} A basic clustering problem in Bayes\-ian statistics is posterior inference in the two-component (symmetric) Gaussian mixture model. More specifically, we will consider that we have data points $b_1,\ldots,b_n \in \mathbb{R}^p$ and we want to sample from the posterior under the following Bayesian model: $u \sim N(0,I_p/p)$, $v \sim \mathsf{Uniform} (\{\pm 1\}^n)$ are the latent cluster assignments and independently 
% $b_i \sim N(v_i \sqrt{\mu/n}\ u, I_p/p)$.
% In other words, we posit that the data points were generated by a balanced mixture of two spherical Gaussians with means $\pm \sqrt{\mu/n}\ u$ and $u$ itself is sampled from a Gaussian distribution. (For simplicity, we assumed that the data is scaled and centered so that the variance of the components is $I_p/p$; the scalings here are chosen in part to maintain consistency with the next example.)  In this case, the posterior on the cluster assignments $v$ is given by $p(v \mid b) \propto \exp\left(\frac{p \mu}{2n(1 + \mu)} \langle vv^\top , BB^\top  \rangle\right)$ 
% where $B \in \R^{n \times p}$ is the matrix with rows $b_i$. (See Appendix~\ref{a:example} for the derivation.) Note that this is an Ising model with
% $ J = \frac{p \mu}{2n(1 + \mu)} BB^\top  $
% and the rank of $J$ is at most $p$. Hence, our main result lets us sample from this distribution (posterior in the Gaussian Mixture Model) in polynomial time in fixed dimension $p$. In the case of a balanced mixture, the posterior will always be bimodal due to the symmetry of swapping the two cluster assignments, and so Glauber dynamics would not be expected to mix. (Also, our algorithms works for general data points $b_1,\ldots,b_n$ in which case the posterior can be an arbitrary positive semidefinite Ising model of rank $p$ --- in particular, it could be a Hopfield network and have even more than two modes.) In fact, the Hubbard-Stratonovich transform and our algorithm as a whole has a natural interpretation in terms of searching over the latent vector $u$ in this case (see Appendix~\ref{app:equiv}).
% %Note that the $\mu$ is exactly the variable appearing in the Hubbard-Stratonovich transform, so algorithm has the natural interpretation of iterating over a grid of $\mu\in \R^p$ (see Appendix~\ref{app:equiv}). \fnote{this $\mu$ is not $\mu$ as defined above, which is just a number?}
% Finally, we note that this example can be easily generalized to assymetric mixture (mixing weights not 50/50); this just changes the prior, which results in an external field in the (Ising model) posterior. 

% \begin{rem}
% Importantly, the posterior sampling result we establish does not rely on the data being a typical sample from the posited Bayesian model. This is useful because in many machine learning and statistics applications the data is not exactly generated from the posited model, and nevertheless sampling from the posterior is very useful. On the other hand, if the data is indeed generated from the model (i.e., well-specified) then posterior sampling lets us compute the Bayes-optimal estimator of quantities of interest, e.g., compute $\Pr(v_i = v_j \mid B)$ in the GMM example which is the Bayes-optimal estimate of $1(v_i = v_j)$, the indicator that $i$ and $j$ are from the same component.  
% %% May not be true in as strong as a sense is hoped.
% %If we assume the data is actually generated from the model, then we can show the naive mean-field approximation becomes accurate as we obtain more data, and so for the posterior and so give a faster algorithm for approximately sampling from the posterior --- see Appendix~\ref{apdx:?}. 
% \end{rem}
% %\fnote{can easily modify to be an unbalanced mixture, also should add in scaling for variance?}
% %\fnote{add example of low-dimensional GMM first?}
% %\fnote{gap they establish is $1/\gamma^{3/2}$, is this gonna be useless if $p = O(1)$? Maybe we can still do $p = o(n)$? Also minor fixme: our $B$ is the transpose of theirs}
% %\fnote{when $p = 1$ and $\lambda = 0$, threshold for weak recovery in one dimension is not $\mu^2/n > 1$ but more like $\mu/n > 0$? because for 1d mixture of gaussians, we need a constant separation for clustering (as opposed to recovering the mean). it's indeed a different regime, should include 1d experiment to illustrate}

% \paragraph{Posterior in Low-Dimensional Contextual SBM.}
% The contextual stochastic block model \citep{deshpande2018contextual} is a more complex version of the previous GMM model in which the cluster structure is also reflected in the community structure of a graph. We consider the low-dimensional version of this model where the dimension of the contexts $p$ is small---this is morally related to, but different from, the spiked Wishart model with side information, see e.g., \cite{montanari2021estimation}. %, though not the same.
% For simplicity, we describe the Gaussianized version of this model below, though our results also apply analogously to the original SBM version. 

% % Deshpande, Montanari, Mossel and Sen \cite{deshpande2018contextual} (see also follow up work) studied the following model for community detection/clustering. 
% The generative model is $v \sim \mathsf{Uniform} (\{\pm 1\}^n)$, $u \sim N(0,I_p/p)$, $W$ is a GOE matrix, i.e., a symmetric matrix where independently $W_{ij} \sim N(0,1/n)$ for $i < j$ and $W_{ii} \sim N(0,2/n)$, and $Z \in \R^{ n \times p}$ is a matrix with iid $N(0,1/p)$ entries. Then we observe
% \[ A = \frac{\lambda}{n} vv^\top  + W, \qquad B = \sqrt{\frac{\mu}{n}} v u^\top  + Z, \qquad u \sim N(0,I_p/p). \]
% Informally, words $A_{ij}$ is some indication of whether $v_i$ and $v_j$ are likely to agree, and rows of $B$ are context/feature vectors in $\mathbb{R}^p$
% from a mixture of two spherical gaussians with means $\pm \sqrt{\mu/n}\ u$, where each gaussian corresponds to one community assignment.
% In this model, the posterior (see Appendix~\ref{a:example} for the derivation) is
% $p(v \mid A,B) \propto \exp\left(\frac{\lambda}{2} \langle vv^\top , A \rangle + \frac{p\mu}{2n(1 + \mu)}\langle vv^\top , BB^\top  \rangle \right)$,
% so it is an Ising model where the interaction matrix is the weighted sum of $A$ and $BB^\top $. We can sample from this using our result as long as the dimension $p$ is fixed (since $BB^\top $ is rank at most $p$) and provided $\lambda\|A\|_{\op} < 1/2$. Note that if $A$ is actually generated from the model, then $\|A\|_{\op} \le 2(1 + o_{n \to \infty}(1))$ due to well-known results on spiked Wigner matrices (see \cite{perry2018optimality} and references within)
% %by classical results \cite{anderson2010introduction} 
% in which case we would have mixing for $\lambda < 1/4$. Like our previous application, the sampler works fine with any context matrix $B$. 

% %Although they studied $p$ proportional to $n$, we can consider also $p$ of order $1$ i.e., low-dimensional contexts. In this case, it seems we should actually take $\mu$ on the order of $n$, which is different from what would naively predict from the proportional scaling setting. The reason is that in 1 dimension, we need a constant separation to achieve nontrivial clustering in a gaussian mixture model (whereas the threshold for recovering the planted direction $u$ is smaller). 
% %% THIS WAS WRONG, it's a ifferent behavior
% %in which case we should take $\mu^2$ on the same order as $n$. NOTE: the trick we use to decompose into mixture of Ising models is exactly the opposite of the integration over $u$ above. 

% %TODO: check that when $\mu^2 = \Theta(n)$, having $A$ in addition to $B$ is useful for estimating e.g., $vv^\top $. (Seems reasonably likely?) 


% %\printbibliography
% \bibliography{bib}

% \appendix

% %\section{Appendix}

% \section*{Overview of Appendix}
% The Appendix includes complete proofs of all of the main results. We set out notations and definitions in Appendix~\ref{a:not-df}. 
% Appendix~\ref{sec:negdef} formalizes the argument for handling negative outlier eigenvalues. Appendix~\ref{sec:Z} gives the proof of the part of Theorem~\ref{t:main} for estimating the partition function, and Appendix~\ref{s:sampling} gives the proof for sampling. 
% Appendix~\ref{app:equiv} provides a re-interpretation of the Hubbard-Stratonovich transform in terms of Gaussian mixture posteriors, and 
% %Appendices~\ref{app:equiv} and 
% Appendix~\ref{app:technical} contains supporting technical lemmas for the previous sections. Appendix~\ref{a:example} contains additional calculations related to the examples. Finally, we prove the computational hardness results in Appendix~\ref{s:hardness}.  
% \section{Notation and definitions}
% \label{a:not-df}
% \subsection{Notation}
% For a set $I\subeq A$, we let $I\cdot c := \set{cx}{x\in I}$; for instance, $\wh Z\in Z \cdot [\rc 2,2]$ means $\rc 2 Z\le \wh Z\le 2Z$.

% We will often omit subscripts and superscripts for probability distributions; when we need to be precise, we will indicate the variables as superscripts (for example, $p^{\si,\mu}$, $p^{\si|\mu}$). We use a lowercase letter $p$ to denote the probability density functions and an uppercase letter $P$ to denote the corresponding probability measure.
% All probability densities are with respect to the uniform measure on the hypercube and Lebesgue measure on $\R^n$. When we write $\propto$, the constants of proportionality do not depend on the variables to the left of the conditioning. 

% \input{notations}

% \subsection{Background on Markov chains}

% \label{a:def}
% Let $P$ be a measure on some space $\Om$ and $T$ be the transition kernel of the ``natural" Markov chain associated with $P$, e.g., Glauber dynamics (Algorithm~\ref{a:mc}) when $P$ is defined on the hypercube $\Om = \{\pm 1\}^n$. 
% The Poincar\'e and modified log-Sobolev constants of  $P$ are defined as
% \begin{align*}
%     \CP(P) &=  \sup\set{\fc{\Var_P(f)}{\cE_P(f,f)}}{f:\BC\to \R, \Var_P(f)\ne 0}\\
%     \CMLS(P) &= \sup\set{\fc{2\Ent_P(f)}{\cE_P(f,\log f)}}{f:\BC\to \R_{\ge 0}, \Ent_P(f)\ne 0}
% \end{align*}
% where $\Ent_P(f) = \E_P[f\log f] - \E_P[f]\log \E_P[f]$, and
% \begin{align*}
%     \cE_P(f,g) &= \E_P[f \cdot \cL_Pg]\\
%     \text{where}\quad \cL_Pf &= (\id - T)f.
% \end{align*}
% In particular, for Glauber dynamics on $\BC$,
% \begin{align*}
% \quad (\cL_Pf)(\si) &=\rc n \sumo in \pa{\E_P[f(x)|x_{-i}=\si_{-i}] - f(\si)}.
% \end{align*}
% Here, for $\si\in \BC$, $\si_{-i}\in \{\pm1\}^{n-1}$ denotes all coordinates except the $i$th one.
% Note that some texts use instead the reciprocal of $\CP,\CMLS$, or do not include the $\rc n$.

% We also define the Cheeger constant of the Markov chain by 
% \begin{align*}
% \Phi &= \min_{A\subeq \Om,P(A)\le \rc 2} \fc{Q(A,A^c)}{P(A)}\\
% \text{where}\quad Q(A,B) &= \int_{A} T(x,B) \,P(dx).
% \end{align*}

% \input{negdef}
% \input{Z}
% \input{sampling}
% \input{equiv2}
% \input{appendix}
% \input{hardness}
% \end{document}



==> old-alg.tex <==

\section{[OLD] Estimating the partition function}

For a PSD matrix $A$, let $\rank_\tau(A)$ denote the number of eigenvalues of $A$ that are $\ge \tau$. Note that $\rank_1(A)\le \ve{A}_F^2$.
\begin{thm}
Suppose $J$ is PSD. 
There is a algorithm that with probability $\ge 1-\de$ outputs an $\ep$-approximation to $Z_{J,h}$, 
\begin{align*}
e^{-\ep} \wh Z_{J,h} \le \wh Z_{J,h} &\le e^\ep \wh Z_{J,h}
\end{align*}
in time $\fc{(\ve{J}_2n)^{O(1+\rank_1(J))}\log\prc \de}{\ep^2}$.
\end{thm}

% \subsection{Counting-to-sampling reduction}

% We use a standard sampling to counting reduction, which expresses the partition function as a product of $n$ ratios. An alternative approach is to introduce a temperature parameter; with an adaptive temperature schedule, only $\wt O(\sqrt n)$ levels are necessary~\cite{vstefankovivc2009adaptive}. \hlnote{We may have to use the annealing approach for sampling anyway.}

% For estimation of $Z_{G,\be, h}$ (Algorithm~\ref{a:counting}), to see that the product $e^{-H_{\be, h}(\si)} \prod_{i=1}^n r_i$ gives the right answer, note that if $p_{v_i}^*$ are the actual probabilities,
% \begin{align*}
%     r_i^* :&= \begin{cases}
%     \rc{p_{v_i}^*}, & \si_i=1\\
%     \rc{1-p_{v_i}^*}, & \si_i=-1
%     \end{cases}
%     \\
%     &= p(\si_i' = \si_i | \si_j' = \si_j \text{ for }j<i) = 
%     \fc{p(\si_j'=\si_j \text{ for } j\le i-1)}{p(\si_j'=\si_j \text{ for } j\le i)}.
% \end{align*}
% Then we have a telescoping product
% \begin{align*}
%     e^{-H_{\be, h}(\si)} \prod_{i=1}^n r_i^*
%     &= 
%     Z_{G,\be, h} \cdot p(\si) \prod_{i=1}^n \fc{p(\si_j'=\si_j \text{ for } j\le i-1)}{p(\si_j'=\si_j \text{ for } j\le i)} = Z_{G,\be, h}.
% \end{align*}
% With appropriate choice of $c$, we can ensure that for each $i$, with probability at least $1-\de/n$, that 
% $p_{v_i}\in [p_{v_i}^* e^{-\fc{\ep}{2n}}, p_{v_i}^* e^{-\fc{\ep}{2n}}]$ and 
% $r_i\in [r_i^* e^{-\ep/n}, r_i^* e^{\ep/n}]$. Then with probability at least $1-\de$, the estimate will be contained in $r_i\in [Z_{G,\be, h} e^{-\ep}, Z_{G,\be, h} e^{\ep}]$.
%  \begin{algorithm}[h!]
%  \label{a:sampling-counting}
%  \caption{Approximation of partition function given sampling algorithm} 
%  \begin{algorithmic}[1] %\label{a:sampling-counting}
%  \Require Algorithm to approximately sample from all conditional distributions $p(\si_{i:n}|\si_{1:i-1})$.
%  \Ensure Approximation of partition function $Z=\sum_{\si\in \{\pm1\}^n}\wt p(\si)$.
%  \medskip  
%  \For{$i = 1 \to n$} 
%  	\State Draw approximate samples $X_{i,j}\in \{\pm 1\}^{\{i,\ldots, n\}}$ from $p(\si_{i:n}|\si_{1:i-1})$.
%  	\State Let $\wh p_i = \rc N |\set{j}{(X_{i,j})_i=1}|$.
%  	\If{$\wh p_{i}\ge \rc 2$}
%  		\State Set $\si_i=1$ and $\wh r_i = \fc{1}{\wh p_{v_i}}$.
%  	\Else
%  		\State Set $\si_i=-1$ and $\wh r_i = \fc{1}{1-\wh p_{v_i}}$.
%  	\EndIf
%  \EndFor
%  \State \Return $\wt Z = \wt p(\si) \prod_{i=1}^n r_i$. 
%  \end{algorithmic}
%  \label{a:counting}
%  \end{algorithm}
 
% \begin{thm}
% There are constants $c_1,c_2$ such that the following holds.
% Let $0<\ep, \de<\rc 2$. In Algorithm~\ref{a:sampling-counting}, suppose that
% $N\ge \fc{c_2\sqrt{\log\prc\de}}n$ and
% $X_{i,j}\sim \wh p(\si_{i:n}|\si_{1:i-1})$ are independent samples form a distribution with 
% \[
% \ve{\wt p(\cdot|\si_{1:i-1}) - p(\cdot |\si_{1:i-1})} \le \fc{c_1\ep}n.
% \]
% Then with probability $\ge 1-\de$, the output of the algorithm $\wt Z$ satisfies
% \[
% e^{-\ep} Z \le \wt Z \le e^{\ep}Z.
% \]
% \end{thm}

\subsection{Algorithm}

Given a probability distribution $p$ on $\{\pm 1\}^n\times B$ where $B\subeq \R^r$, we can define the Markov chain in Algorithm~\ref{a:mc}. Let $\si^{(i)}=(\si_1,\ldots, -\si_i, \ldots, \si_n)$ denote $\si$ but with the $i$th coordinate flipped.

 \begin{algorithm}[h!]
 \caption{Markov chain on $\{\pm 1\}^n\times B$} 
 \begin{algorithmic}[1]
 \Require Query access to probability distribution $p(\si,x)$ on $\{\pm 1\}^n\times B$, up to constant of proportionality; method to sample the conditional distribution $p(x|\si)$; number of steps $T$.
 \Ensure Approximate sample from $p$.
 %Approximation of partition function $Z_{J,h}$.
 \For{$1\le t\le T$} 
    \Block{With probability $\rc 2$,}
        \State Choose a random coordinate $i$, and set $(\si,x) \leftarrow (\si^{(i)},x)$ with probability $\fc{p(\si^{(i)},x)}{p(\si^{(i)},x)+p(\si,x)}$.
    \EndBlock
    \State Sample $y\sim p(\cdot |\si)$, and set $(\si,x)\leftarrow  (\si,y)$.
 \EndFor
 \end{algorithmic}
  \label{a:mc}
 \end{algorithm}

% Let $(\si, x)$ denote the current state. Let $\si^{(i)}=(\si_1,\ldots, -\si_i, \ldots, \si_n)$ denote $\si$ but with the $i$th coordinate flipped.
% \begin{enumerate}
%     \item For every $i$, with probability $\rc{2(n+1)}$, propose a transition to $(\si^{(i)}, x)$, and accept with probability $\fc{p(\si^{(i)},x)}{p(\si^{(i)},x)+p(\si,x)}$.
%     \item With probability $\rc{2(n+1)}$, choose $y\in B$ uniformly, propose a transition to $(\si,y)$, and accept with probability $\fc{p(\si,y)}{p(\si,y) + p(\si,x)}$.
% \end{enumerate}
% Up to constants, the spectral gap of this Markov chain is the same as the spectral gap for the Markov process with generator defined as 
% \begin{align*}
%     \sL f(\si,x)
%     &= \sumo in \fc{p(\si^{(i)},x)}{p(\si^{(i)},x)+p(\si,x)} (f(\si^{(i)}, x) - f(\si,x))\\
%     &\quad 
%     + \rc{\Vol(B)} \int_{B} \fc{p(\si,y)}{p(\si,y) + p(\si,x)}(f(\si,y)-f(\si,x))\,dy
% \end{align*}
% and Dirichlet form
% \begin{align*}
%     \sE f(\si,x) &= 
%     \E_p\ba{
%         \sumo in \pa{f(\si,x) - \E_p [f(\si,x)|\si_{-i}, x]}^2 + 
%         \rc{\Vol(B)} \int_B \pa{f(\si,x) - \E_p [f(\si,x)|\si]}^2
%     },
% \end{align*}
% where $\si_{-i}$ denotes $\si$ with the $i$th coordinate omitted.
% \fixme{(Details.)}

Our algorithm is then given by Algorithm~\ref{a:Z}. 
%\hlnote{Not quite right: need to figure out $p(\mu^\prl)$. The algorithm requires discretization $\eta$ depending on $\ep$ getting $1/\ep$ factors inside the base. To only suffer $\ep^2$, need to run a Markov chain in the slice---alternate $\si$ and $\mu$.}

%\hlnote{If we don't care about constants in the exponent, OK to restrict to $\log(1/\ep)$-sized ball, because $\log(1/\ep)^{\rank_1(A)} = O(n^{\rank_1(A)})$ for $\ep>2^{-n}$, and for $\ep\le 2^{-n}$, can brute force.}

 \begin{algorithm}[h!]
 \caption{Approximating partition function of Ising model} 
 \begin{algorithmic}[1]  
 \Require Discretization $\eta$, length $L$.
 \Ensure Approximation of partition function $Z_{J,h}$.
 \State Factor $J=\rc n XX^\top$ for $X\in \R^{n\times n}$.
 \State Let $V$ denote the subspace of $\R^n$ spanned by the eigenvectors of $J$ with eigenvalues $>1$. Let $P^\prl$ and $P^\perp$ the projections to $V$ and $V^\perp$. Let $Q\in \R^{n\times r}$ be the matrix with columns that are an orthonormal basis for $V$.
 \medskip  
 \For{$i_1,\ldots, i_r \in \bc{-\fc L\eta, -\fc L\eta+1,\ldots, \fc L\eta-1}$} 
 	\State Let $B_i = \prod_{j=1}^r [i_j \eta, (i_j+1)\eta]$. %and $y_i$ be the center of this cube.
 	\State Obtain an estimate $\wt Z_i$ of \[Z_i:= 
 	\int_{y\in B}
\sum_{\si\in \{\pm 1\}^n}
\exp\pa{\rc{2} \si^\top \pf{X^\top P^\perp X}n \si 
    + \sumo in \pa{-\rc 2 \ve{\si_i P^\prl x_i - Qy}^2 + h_i\si_i}}
 	\]
 	%Z_{\rc nX^\top P^\perp X, h+P^\prl \nu_i}$ 
 	by using Algorithm~\ref{a:sampling-counting} with the sampling algorithm being %Glauber dynamics 
 	the Markov chain \fixme{defined above} 
 	run for $Cn^2\log \pf{n}{\ep}$ steps (for large enough constant $C$).
 \EndFor
 \State  %\Return $\wt Z = \eta^r \sum_{i\in \bc{-\fc L\eta, -\fc L\eta+1,\ldots, \fc L\eta-1}^r} \wt Z_i$. 
 Return $\wt Z =  \exp\pa{-\rc 2 \ve{P^\prl X}_F^2}
 \sum_{i\in \bc{-\fc L\eta, -\fc L\eta+1,\ldots, \fc L\eta-1}^r} \wt Z_i$.
 \end{algorithmic}
  \label{a:Z}
 \label{a:counting}
 \end{algorithm}
 
% To analyze this algorithm, we use a decomposition theorem similarly to~\cite{otto2007new,ge2018simulated}.

% \begin{thm}

% \end{thm}
\hlnote{Easier to analyze when we integrate out $x\in B$. (This is just integral of a Gaussian over a box.)}

We show mixing of this chain by comparison to Glauber dynamics on the marginal distribution of $\si\in \{\pm 1\}^n$. \fnote{shouldn't it be modified log-sobolev constant here?} \hlnote{Yes, fixed.}

\begin{lem}
Suppose $\eta = O\prc{nLr + n\ve{J}_2 \sqrt r}$.
The marginal distribution of $\si$ of 
\[
p_{X,h,V}(\si,y)\propto  
\exp\pa{\rc{2} \si^\top \pf{X^\top P^\perp X}n \si 
    + \sumo in \pa{-\rc 2 \ve{\si_i P^\prl x_i - Qy}^2 + h_i\si_i}}
\]
over $\{\pm 1\}^n \times B_i$
has modified log-Sobolev constant bounded by $O(n)$, and Glauber dynamics %on the marginal distribution 
mixes in time $O(n^2\log n)$. 
\end{lem}
Note that we can run this chain, as we can numerically integrate \[\int_B \pf{n}{2\pi}^{\fc n2} \exp\pa{-\fc n2 \ve{\mu^\prl - \fc{\sumo in \si_i P^\prl x_i}n}^2}\,d\mu^\prl \]
as this is a product distribution in $\mu^\prl$. However, it will be more elegant to consider an algorithm which alternately resamples $\si$ and $\mu$.

\begin{proof}
Let $J^\perp = \rc n X^\top P^\perp X$, and for a symmetric matrix with diagonalization $A=UDU^\top$, let $D_{\le \tau}$ denote $D$ with the entries $\ge \tau$ replaced by $\tau$, and $A_{\le \tau} := UD_{\le \tau} U^\top$.
Let $y_i$ be the center of $B_i$. By Lemma~\ref{l:joint-prl}
\[
p_{X,h,V}(\si | y_i)\propto 
\exp\pa{\rc 2 \si^\top J^\perp \si + (h+X^\top Qy_i)^\top \si}.
\]
By~\cite[Theorem 12]{anari2021aentropic}, the modified log-Sobolev constant for 
\[
p_{(J^\perp)_{\le 1-\rc n}, h+X^\top Qy}(\si)\propto 
\exp\pa{\rc 2 \si^\top (J^\perp)_{\le 1-\rc n} \si + (h+X^\top Qy)^\top \si}.
\]
is bounded by $\pa{1-\ve{(J^\perp)_{\le 1-\rc n}}}^{-1} = n$. Since 
\begin{align}\label{e:gibbs-r1}
\ab{\log \fc {p_{X,h,V}(\si | y_i)}{p_{(J^\perp)_{\le 1-\rc n}, h+X^\top Qy}(\si)}}
\in 
\rc 2 \ve{J^\perp - (J^\perp)_{\le 1-\rc n}}_F\sqrt n \cdot [-1,1] = \ba{-\rc 2, \rc 2}.
\end{align}
Moreover, we have 
\begin{align}\label{e:gibbs-r2}
    \ab{\log \fc{p_{X,h,V}(\si | y\in B)}{p_{X,h,V}(\si | y_i)}} \in [-O(1),O(1)]
\end{align}
because 
\begin{align*}
&\fc n2 
\pa{\max_{y\in B}
\ve{Qy - \fc{\sumo in \si_i P^\prl x_i}n}^2-
\min_{y\in B}
\ve{Qy - \fc{\sumo in \si_i P^\prl x_i}n}^2
}\\
&\le 
\max_{y_1,y_2\in B}
\ba{\fc n2 \pa{\ve{Qy_1}^2 - \ve{Qy_2}^2} + \an{Q(y_2-y_1), \sumo in \si_i P^\prl x_i}}\\
&\le \fc n2 L\sqrt r \cdot \eta \sqrt r
+ \eta \sqrt r \cdot \ve{P^\prl X}_2\sqrt n\\
&\le \fc n 2 L\eta r + \eta n\sqrt r \ve{J}_2=O(1)
\end{align*}
when $\eta =\rc{nLr + n\ve{J}_2\sqrt r}$.

Combining~\eqref{e:gibbs-r1} and~\eqref{e:gibbs-r2} and using the Holley-Stroock perturbation lemma, the modified log-Sobolev constant for $p_{X,h,V}(\si|y_i)$ is bounded by $O(n)$. 

Finally, the proof of mixing time based on the exchange property (\cite[Lemma 37]{anari2021aentropic}) still goes through under the perturbation, showing the result on mixing time.
\end{proof}
\fixme{Now we compare a chain where we alternatingly resample $\si$ and $\mu$. We consider one step of the chain to be sampling $\mu$, then $\si$. It suffices to consider the marginal distribution on $\si$, since after resampling $\mu|\si$, the $p(\mu|\si)$ has the correct distribution. We claim that the transition probability from $\si$ to $\si_{-i}$ is lower (and upper) bounded by a constant times the transition probability in the Glauber chain on the marginal distribution. }
%In other words, we can consider this process as a ``censored" version of the original chain... 
\begin{lem}\label{l:ls-slice}
Suppose $\eta = O\prc{nLr + n\ve{J}_2 \sqrt r}$.
The alternating Gibbs sampler on 
\[
p_{X,h,V}(\si,y)\propto  
\exp\pa{\rc{2} \si^\top \pf{X^\top P^\perp X}n \si 
    + \sumo in \pa{-\rc 2 \ve{\si_i P^\prl x_i - Qy}^2 + h_i\si_i}}
\]
over $\{\pm 1\}^n \times B_i$
has mixing time bounded by $O(n(n\log (n)+\log \max \ve{h_i}))$.
%has log-Sobolev constant bounded by $O(n)$, and Glauber dynamics %on the marginal distribution 
%mixes in time $O(n(n\log (n)+\max \ve{h_i}...))$. 
\end{lem}
\begin{proof}
After every step involving $y$, for every $\si$, the distribution $p(y|\si)$ is correct. Hence, for computation of mixing time, it is equivalent to consider the following Markov chain on $\{\pm 1\}^n$: draw $p(\si|y)$, propose a move from $(\si,y)$ to $(\si^{(i)},y)$, and then drop $y$. The Dirichlet form of this chain is
\begin{align*}
    \sE_{\textup{alt}}(f) &= \E_{\si\sim p(\cdot|y\in B)}
    \sum_{i=1}^n \E_{y\sim p(\cdot|\si, y\in B)} \fc{p(\si^{(i)},y)}{p(\si^{(i)},y) + p(\si,y)} (f(\si) - f(\si^{(i)}))^2.
\end{align*}
By~\eqref{e:gibbs-r2}, this coefficient is lower-bounded by $\Om(1) \cdot \fc{p(\si^{(i)}|y\in B)}{p(\si^{(i)}|y\in B)+p(\si|y\in B)}$, so 
\begin{align*}
    \sE_{\textup{alt}}(f) &= \Om(1) \cdot  \E_{\si\sim p(\cdot|y\in B)}
    \sum_{i=1}^n \fc{p(\si^{(i)}|y\in B)}{p(\si^{(i)}|y\in B)+p(\si|y\in B)}(f(\si) - f(\si^{(i)}))^2 = \Om(1) \sE(f).
\end{align*}
Hence the modified log-Sobolev constant of this chain is bounded by $O(1)$ times the modified log-Sobolev constant of Glauber dynamics on the marginal distribution, which is $O(n)$. 
The mixing time bound then follows from $\log \log  \rc{\min p(\si|y\in B)} = O(\log n + \log \ve{h_i})$.
\end{proof}

\fixme{We can get rid of $\ve{h_i}$ by arguing that Lemma~\cite[Lemma 22]{anari2021log} still goes through. But we will suffer something like it later on anyway...
}

\subsection{Simulated annealing for partition function estimation}

We show that a non-adaptive temperature schedule of length $O(n)$ is sufficient for partition function estimation. Note that a shorter schedule of length $O(\sqrt n \log n \log \log n)$ is possible, and can be found in $n\polylog(n)$ total queries to approximate sampling oracles %for $p_{\be}$
at the different temperatures~\cite{vstefankovivc2009adaptive}.

\hlnote{I don't know whether there is a fixed schedule of length $O(\sqrt n)$... would need to show subexponential concentration of $\si^\top J\si$ under $p_i$.}

% \begin{lem}
% Let $p_i(\si)\propto \exp(\be_i \si^\top J\si + h^\top \si + c(\si))$. %and suppose $\osc c_i\le C$. 
% Let $g_i = \exp((\be_{i+1}-\be_i) \si^\top J \si)$. 
% Then
% \begin{align*}
%     \fc{\E_{p_i} g_i^2}{(\E_{p_i}g_i)^2} 
%     &\le \exp(2(\be_{i+1}-\be_i)\ve{J}_2 d).
% \end{align*}
% In particular, for a temperature schedule with $\be_{i+1}-\be_i\le \rc{2d\ve{J}_2}$, this is at most $e$.
% \end{lem}
% \begin{proof}
% This follows from noting that 
% \begin{align*}
%     \E_{p_i} g_i^2 &\le \max_{\si\in \{\pm 1\}^d} \exp(\be_i \si^\top J \si) \le \exp(2(\be_{i+1}-\be_i)\ve{J}_2 d)\\
%     \E_{p_i} g_i &\ge 1.
% \end{align*}
% \end{proof}



% \fixme{
% We show that a temperature schedule of length $O(\sqrt n)$ is sufficient for partition function estimation.
% \begin{lem}
% Let $p_i(\si)\propto \exp(\be_i \si^\top J\si + h^\top \si + c_i(\si))$ and suppose $\osc c_i\le C$. Let $g_i = \exp((\be_{i+1}-\be_i) \si^\top J \si)$. 
% \begin{enumerate}
%     \item 
%     Suppose $\be_i\ve{A}_2<1$ and $4(\be_{i+1}-\be_i)\ve{A}_2\sqrt d\le 1$. 
% Then
% \begin{align*}
%     \fc{\E_{p_i} g_i^2}{(\E_{p_i}g_i)^2} 
%     &\le 1 + \fc{16Ce^2d(\be_{i+1}-\be_i)^2}{1-\be_i\ve{A}_2}.
%     %\sfc{1-\be_i \ve{A}_2}{d}.
% \end{align*}
% \item 
% In particular, if 
% \begin{align*}
%     \be_{i+1}\le \be_i + \fc{\sqrt{1-\be_i\ve{A}_2}}{4e\sqrt{Cd}},
% \end{align*}
% then $\fc{\E_{p_i} g_i^2}{(\E_{p_i}g_i)^2} 
%     \le 2$.
% \item
% If $\ve{A}_2\le 1$, taking $\be_t = 1-\pa{\fc{t}{8e\sqrt{Cd}}}^2$ for $0\le t\le 8e\sqrt{Cd}$ and $\be_{\ce{ 8e\sqrt{Cd}}}=1$, we have that $\fc{\E_{p_i} g_i^2}{(\E_{p_i}g_i)^2}  \le 2$ for each $0\le i\le \ce{ 8e\sqrt{Cd}} -1$.
% \end{enumerate}

% \end{lem}
% \fixme{$d$ should be $n$ here.}
% \begin{proof}
% The Poincar\'e constant of $p_i$ is at most $\CP := \fc C{1-\be_i\ve{A}_2}$. Then
% \begin{align*}
%     \Var(g_i) &\le 
%     \CP \E_{p_i} \sumo in \pa{\E_{p_i}[g_i(\si)|\si_{-i}]-g_i(\si)}^2\\
%     &\le \CP \fixme{n?}\max_{\si,1\le j\le n} \pa{g_i(\si)-g_i(\si^{(j)})}^2\\
%     %&\le \CP \max\ve{\nb g_i}^2\\
%     &\le \fc C{1-\be_i\ve{A}_2} \cdot 
%     (e(\be_{i+1}-\be_i)4\sqrt d)^2\\
%     &=\fc{16Ce^2d(\be_{i+1}-\be_i)^2}{1-\be_i\ve{A}_2}.
% \end{align*}
% Dividing by $(\E_{p_i}g_i)^2\ge 1$ then gives part 1. Part 2 follows directly by substitution. \fixme{Part 3 computation.}
% %\fixme{Divide by $(\E g_i)^2$}
% %Rearranging gives the desired inequality.
% \end{proof}}


\begin{lem}\label{l:sched}
Suppose $0<\ep,\de<1$. 
Set the temperature schedule as $\be_k = \fc{k}{2d\ve{J}_2}$ for $k < 2d\ve{J}_2$ and $\be_{\ce{2d\ve{J}_2}}=1$. Let $M=\ce{2d\ve{J}_2}$ be the length of the temperature schedule.
Let $p_i(\si)\propto \exp(\be_i \si^\top J\si + h^\top \si + c(\si))$ and suppose $\wt p_i$ is a distribution such that $d_{\TV}(p_i,\wt p_i)\le \fc{\ep}{4M}$. 
Given $N>\fc{5(e-1)M}{\de \ep^2}$ samples $X_{i,j}\sim \wt p_{i}$  for each $0\le i<M$, form the estimate
\begin{align*}
    Y_i &= \rc N \sumo jN g_i(X_{i,j})
\end{align*}
and let $\wh Z = Z_0\prodz i{M-1} Y_i$, where $Z_0 = \sum_{\si\in \{\pm 1\}^n} \exp(h^\top \si + c(\si))$. 
Letting the actual partition function be $Z=\sum_{\si\in \{\pm 1\}^n} \exp(\si^\top J \si + h^\top \si + c(\si))$, we have 
\[\Pj(\wh Z \nin [1-\ep, 1+\ep] Z)\le \de.\]
\end{lem}

We use the following lemma, which roughly says that when the variance of some random variables are close to 1, then the variance is additive under multiplication.
\begin{lem}[{\cite[Lemma B.2]{ge2020estimating}}]\label{lem:prodvar}\label{l:prod}
    Let $Y_i$, $i = 1, \ldots, M$ be independent variables and let $\bar{Y}_i = \EE Y_i$. Assume there exists $\eta > 0$  such that $\eta M \leq \frac{1}{5}$ and
    \begin{equation*}
        \EE Y_i^2 \leq (1 + \eta) \bar{Y}_i^2,
    \end{equation*}
    then for any $\ep > 0$
    \begin{equation*}
        \mathbb{P}\Biggl( \frac{ \ab{ Y_1 \cdots Y_M - \bar{Y}_1 \cdots \bar{Y}_M}}{\bar{Y}_1 \cdots \bar{Y}_M} \geq \frac{\ep}{2} \Biggr) \leq \frac{5 \eta M}{\ep^2}.
    \end{equation*}
\end{lem}

\begin{proof}[Proof of Lemma~\ref{l:sched}]
First we consider the variance of the estimate. We have
\begin{align}
\label{l:g-var}
\Var_{X_{i,1},\ldots, X_{i,N}\sim \wt p_i}\pa{\rc N \sumo jN g_i(X_j)}
    %\E_{X_{i,1},\ldots, X_{i,N}\sim \wt p_i}\pa{\rc N \sumo jN g_i(X_j)} 
\le 
    \rc N (\osc \exp(2(\be_{i+1}-\be_i)\si^\top J \si))
    %- \min \exp(2(\be_{i+1}-\be_i)\ve{J}_2 d))
    \le \fc{e-1}N. 
\end{align}
Let $\E Y_i = \ol{Y_i}$. 
Since $\ol{Y_i}^2 = (\E_{X\sim \wt p_i}g_i(X))^2$, we obtain that $\E Y_i^2 \le 1+\fc{e-1}N\ol{Y_i}^2$. By Lemma~\ref{l:prod} with $\eta =\fc{e-1}N$ and substituting the value of $N$, 
\begin{align}
\label{e:sched-var}
    \Pj\pa{
        \fc{\ab{\prodz i{M-1} Y_i - \prodz i{M-1}\ol Y_i}}{\prodz i{M-1}\ol Y_i}\ge \eph
    }\le \fc{5(e-1)M}{N\ep^2}
    \le \de.
\end{align}

Now we consider the bias, that is, the error of $\prodz i{M-1}\ol Y_i$.
We have that 
\begin{align*}
    \ab{\ol Y_i - \E_{X\sim p_i} g_i (X)}
    &\le %(\max g_i (\si) - \min g_i (\si))
    (\osc g_i) \cdot 
    d_{\TV} (\wt p_i, p_i)\le (\sqrt e-1) \fc{\ep}{4M}\le \fc{\ep}{4M}.
\end{align*}
Taking a product, we obtain
\begin{align}
\label{e:sched-bias}
    \ab{Z_0\prodz i{M-1} \ol Y_i - Z} &\in \ba{\pa{1-\fc{\ep}{4M}}^M,\pa{1+\fc{\ep}{4M}}^M}\cdot Z.
\end{align}
Putting together~\eqref{e:sched-var} and~\eqref{e:sched-bias}, %and substituting the value of $N$, 
we obtain the conclusion.
\end{proof}
By a standard concentration argument, we can boost the success probability to $1-\de'$ by repeating $\Om\pa{\log \prc{\de'}}$ times for a fixed $\de<\rc 2$ and taking the median.

% \hlnote{(1) Probably it's most straightforward to marginalize coordinates one by one. 
% %Naively we will cut off at some radius $\sqrt{\log \prc \ep}$ and incur a $\log\prc \ep$ factor in the base of the exponent.
% (2) Can get temperature schedule of length $\sqrt n$ with annealing %,
% %and avoid the $\log \prc \ep$, 
% but this is more complicated.}

% Simulated annealing is a standard method to reduce counting problems to sampling problems.

% \begin{thm}
% Suppose we have the following.
% \begin{enumerate}
%     \item 
%     A sequence of distributions $p_i = \fc{\wt p_i}{Z_i}$ on $\Om$, such that letting $r_i (x)= \pf{\wt p_{i+1}(x)}{\wt p_i(x)}^2$,
%     \begin{align*}
%         \fc{\E_{x\sim p_i} r_i^2}{\pa{\E_{x\sim p_i}r_i}^2} &\le 1+...\ep
%     \end{align*}
%     \item 
%     Independent samples $X_{i,j}\sim \wh p_i$ for $1\le i\le L$, $1\le j\le N$, where $\ve{\wh p_i - p_i}_{\textup{TV}}\le ...\ep$. 
%     \item An initial estimate $\wh Z_1$...
% \end{enumerate}
% Then letting 
% \begin{align*}
%     \wh R_i &= \rc N \sumo iN r_i(X_{i,j})\quad \text{and} \quad 
%     \wh Z = \wh Z_1 \prod_{i=1}\wh R_i.
% \end{align*}
% with probability $1-\de$, 
% \begin{align*}
%     e^{-\ep} Z_L \le \wh Z \le e^{\ep} Z_L
% \end{align*}
% \end{thm}

\section{[OLD] Sampling}

% \hlnote{The $\log\prc\ep$ takes some more work to show, doing $\poly\prc\ep$ first}
% \begin{thm}
% Suppose $J$ is PSD. 
% There is a algorithm that outputs a sample from a distribution that is $\ep$-close to $p_{J,h}$ 
% in time $\fc{\ve{J}_2n^{O(1+\rank_1(J))}\log\prc \ep}{\ep^2}$.
% \end{thm}

Denote the approximately normalized probabilities
\begin{align*}
    q_{\ell,i}(\si,\mu^\prl) 
    & = \pf{\eta}{L}^n \rc{Z_{\ell, i}} \exp\pa{\rc{2}\be_\ell  \si^\top \pf{X^\top P^\perp X}n \si 
    + \sumo in \pa{-\rc 2 \ve{\si_i P^\prl x_i - \mu^\prl}^2 + h_i\si_i}}.
\end{align*}

We define a Markov chain on an expanded state space $\{0,\ldots, M\} \times [-L,L]^n \times \{\pm 1\}^n$, where the first index denotes the ``temperature" of the distribution. This is similar to a simulated tempering chain~\cite{marinari1992simulated}, with two types of moves: between temperatures and within temperatures. There are two differences with a standard simulated tempering chain:
\begin{enumerate}
    \item We use a different normalizing constant $Z_{\ell, i}$ within each box, in order to make sure the stationary distribution is roughly uniformly distributed over the boxes.
    \item Within any temperature other than the highest one, we only allow a move that stays within the current box.
\end{enumerate}
We need these for technical reasons to make our proof work; it is an interesting question whether a standard simulated tempering chain would work. Our proof strategy is similar to~\cite{ge2018simulated}.

%Consider the following chain on $\{0,\ldots, M\} \times [-L,L]^n \times \{\pm 1\}^n$. 
We define the Markov chain on $\{0,\ldots, M\} \times [-L,L]^n \times \{\pm 1\}^n$ as follows. At each step,
\begin{enumerate}
    \item With probability $\rc 4$, if $\ell \ne M$, propose a move to $(\ell+1,\mu_{\prl},\si)$ and accept with probability $\min\bc{\fc{q_{\ell+1}(\mu_\prl,\si)}{q_\ell(\mu_\prl,\si)},1}$.
    \item With probability $\rc 4$, if $\ell \ne 0$, propose a move to $(\ell-1,\mu_{\prl},\si)$ and accept with probability $\min\bc{\fc{q_{\ell-1}(\mu_\prl,\si)}{q_\ell(\mu_\prl,\si)},1}$.
    \item 
    With probability $\rc 2$, resample $q_\ell(\si|\mu_\prl)$.
    \item 
    In any of the cases: 
    If $\ell\ne 0$, resample $q_\ell(\mu_\prl\in \redd{B(\mu_\prl)}|\si)$. If $\ell=0$, resample $q_0(\mu_\prl\in [-L,L]^n|\si)$. 
\end{enumerate}


\begin{thm}\label{t:samp}
Suppose $J$ is PSD. 
There is a algorithm that outputs a sample from a distribution that is $\ep$-close to $p_{J,h}$ 
in time $\ve{J}_2n^{O(1+\rank_1(J))}\log\prc\ep$.
\end{thm}
%We use the following decomposition theorem for Markov chains.
Given a Markov chain on $\Om$, we define two Markov chains associated with a partition of $\Om$.
\begin{df}\label{df:assoc-mc}
For a Markov chain $M=(\Om, P)$, and a set $A\subeq \Om$, define the \vocab{restriction of $M$ to $A$} to be the Markov chain $M|_A = (A, P|_{A})$, where
$$
P|_A(x,B) = P(x,B) + \one_B(x) P(x,A^c).
$$
(In words, $P(x,y)$ proposes a transition, and the transition is rejected if it would leave $A$.)

Suppose the unique stationary distribution of $M$ is $p$. 
Given a partition $\cal P = \set{A_j}{j\in J}$, define the \vocab{projected Markov chain with respect to $\cal P$} to be $\ol M^{\cal P} = (J, \ol P^{\cal P})$, where
$$
\ol P^{\cal P} (i,j) = 
%\rc{\mu(A_i)} \int_{A_i}\int_{A_j} P(x,dy)\mu(dx).
\rc{p(A_i)} \int_{A_i}\int_{A_j} P(x,y)p(x)\dx.
$$
(In words, $\ol P(i,j)$ is the ``total probability flow'' from $A_i$ to $A_j$.)

We omit the superscript $\cal P$ when it is clear.
\end{df}

The following theorem lower-bounds the gap of the original chain in terms of the gap of the projected chain and the minimum gap of the restricted chains.
\begin{thm}[\cite{madras2002markov}]
\label{t:decomp}
Let $M=(\Om, P)$ be a Markov chain with stationary distribution $p$. Let $\cal P=\set{A_j}{j\in J}$ be a partition of $\Om$ such that $p(A_j)>0$ for all $j\in J$. Then 
\begin{align*}
    \rc 2 \Gap( \ol M^{\cal P}) \min_{j\in J} \Gap (M|_{A_j}) &\le \Gap(M) \le \Gap(\ol M^{\cal P}).
\end{align*}
\end{thm}
\begin{proof}[Proof of Theorem~\ref{t:samp}]
Below, we condition on the event that all the $Z_{\ell,i}$ are $2$-multiplicative approximations. Choosing the failure probability to be $O\pa{\ep \rc M \pf{\eta}{L}^n}$, this event happens with probability $1-O(\ep)$. 

We first claim that $1-O(\ep)$ of the probability mass of $p(\si,\mu^\prl)$ is contained in $[-L,L]^n$. For this, it suffices to fix $\si$, and show that $p(\mu^\prl \nin [-L,L]^n|\si) = O(\ep)$. We have
\[
p(\mu^\prl |\si) = \pf{n}{2\pi}^{n/2} \exp\pa{-\fc n2 \ve{\mu^\prl - \fc{\sumo in \si_i P^\prl x_i}n}^2}.
\]
Note
\[
\ve{\fc{\sumo in \si_i P^\prl x_i}n} \le \ve{\fc{X^\top P}{n}}_2 \sqrt n \le \sqrt{n \ve{J}_2}.
\]
Hence taking 
\[
L = \sqrt{n\ve{J}_2} + \Om\pa{\sqrt n \log \pf n\ep},
\]
we have
\[
\Pj(\mu^\prl \nin [-L,L]^n) \le \sumo in \Pj((\mu^\prl)_i\nin [-L,L]) = nO\pf \ep n = O(\ep).
\]
Thus \[d_{\TV} (p,p|_{\{\mu\in [-L,L]^n\}}) = O(\ep).\]

We use Theorem~\ref{t:decomp} with the partition given by $A_{\ell,i}= \{\ell\}\times B(i) \times \{\pm 1\}^n$. Given that $\wt Z_{\ell,i}\in [1-O(\ep), 1+O(\ep)]\cdot Z_{\ell,i}$, we have that
\[
d_{\TV} \pa{p|_{\{\mu\in [-L,L]^n\}}, 
\sumz \ell M\sum_{i\in \{-\fc L\eta, \ldots, \fc L\eta - 1\}^n} \fc{\wt Z_{\ell,i}}{Z_{\ell,i}} p\one_{\{\ell\}\times B_i\times \{\pm 1\}^n}
} = O(\ep). 
\]
The restriction $M|_{A_{\ell,i}}$ is exactly the lazy chain we defined on $q_{\ell,i}$, which has Poincar\'e constant bounded by $O(n)$ by Lemma~\ref{l:ls-slice}. 

For the projected chain, we use Lemma~\ref{l:proj}. We check each of the conditions.
\begin{enumerate}
    \item By Lemma~\ref{l:g-var}, $\chi^2(q_{\ell+1,i}||q_{\ell,i}) = O(1)$ so $d_{\TV}(q_{\ell+1,i}||q_{\ell,i}) = 1-\Om(1)$ in the projected chain $\ol M$, 
    \begin{align*}
        P((\ell,i), (\ell\pm 1,i)) &=\Om\pa{\min\bc{\fc{P((\ell\pm 1, i))}{P((\ell, i))},1}}\\
        P((0,i), (0,j)) &= \Om(q_0(B(j)).
    \end{align*}
    \item To bound the ``bottleneck ratio", note that for $k<\ell$, $\fc{q_k(B(i))}{q_\ell(B(i))} = \Om\pa{\pf \eta L^d}$. 
    \item Under the event that the estimates of the partition functions are accurage, 
    \[
    P\pa{\{\ell\} \times \bc{-\fc L\eta, \ldots, \fc L\eta-1}^d \times \{\pm 1\}^n} = \Om\prc M. 
    \]
    Hence by the Lemma, the Poincar\'e constant of the projected chain is $O(M^2)$.
\end{enumerate}
 Noting the spectral gap is the inverse of the Poincar\'e constant and using Lemma~\ref{t:decomp}, we get that the Poincar\'e constant of $M$ is $O\pa{M^2 \pf{L}{\eta}^d n^2} = O\pa{\pf{L}{\eta}^d n^4}$. % This gives the desired bound.
 Taking $L=\sqrt{n\ve{J}_2} + \Te\pa{\sqrt n \log \pf n\ep}$ and $\eta = \Te \prc{nLr + n\ve{J}_2\sqrt r}$, the total mixing time is $\pa{n\pa{\ve{J}_2 + \log \pf 1\ep}}^{O(d)}\log \prc \ep$.
% \fixme{Mixing time}
\end{proof}

==> old.tex <==
\subsection{Analysis of simple estimator}
Let $S_n$ denote the unit sphere in $n$ dimensions, noting that this is different from the convention in \cite{deshpande2018contextual} where the sphere is scaled by $\sqrt{n}$.
%\fnote{Notational comparison. They use a rescaled unit sphere everywhere...}
\fnote{move to appendix in final version}
In \cite{deshpande2018contextual} they analyze the following simple estimator (Equations 25-26) using Gaussian comparison inequalities:
\begin{align*}
T_{n,p}(A,B) := \max_{x \in S_n, y \in S_p} \left[\langle x, A x \rangle + b_* \langle x, B y \rangle\right]
\end{align*}
Substituting in the definition of $A$ and $B$, observe that
\[ T_{n,p} =  \max_{x \in S_n, y \in S_p} \left[\frac{\lambda}{n} \langle x, v \rangle^2 + \langle x, W x \rangle + b_* \sqrt{\frac{\mu}{n}} \langle x, v \rangle \langle u, y \rangle + b_* \langle x, Z y \rangle \right]. \]
It was observed by \cite{deshpande2018contextual} this optimization problem can be upper and lower bounded by two different optimization problems, which are more tractable because they both eliminate the term $b_* \langle x, Z y \rangle$.
%FIX: looks like there are various typos in their paper, just do the calculations explicitly.
\begin{lem}[Proposition 13 of \cite{deshpande2018contextual}]\label{lem:prop13}
Conditional on $u,v$ (i.e. taking expectation over $W,Z$ only) we have
\begin{align*}
    \E_{W,Z} T_{n,p} &\le \E_{g,h} \max_{x \in S_n, y \in S_p} \left[\frac{\lambda}{n} \langle x, v \rangle^2  + \langle x, g \rangle + b_*\sqrt{\frac{\mu}{n}} \langle x, v \rangle \langle y, u \rangle + \langle y, h \rangle\right]
\end{align*}
where $g \sim N(0, \frac{4 + b_*^2n/p}{n} I_n)$ and $h \sim N(0, \frac{b_*^2}{p} I_p)$ independent of everything else, 
and
\begin{align*}
    \E_{W,Z} T_{n,p} &\ge \E_{D,E} \max_{x \in S_n, y \in S_p} \left[\frac{\lambda}{n} \langle x, v \rangle^2 + \langle x, D  x\rangle + b_*\sqrt{\frac{\mu}{n}} \langle x, v \rangle \langle y, u \rangle + \langle y, E y \rangle  \right]
\end{align*}
where $D_{ij} \sim N(0, (1 + b_*^2n/4p)/n)$ for $i < j$ and $D_{ii} \sim N(0, 2(1 + b_*^2n/4p)/n)$ is a symmetric random matrix, and similarly $E_{ij} \sim N(0, b_*^2/4p)$ and $E_{ii} \sim N(0, b_*^2/2p)$.
\end{lem}
\begin{proof}
This proof is taken from \cite{deshpande2018contextual}; we repeat it for the reader's convenience, because we use slightly different notation. It uses the Sudakov-Fernique inequality for maxima of non-centered Gaussian processes, see e.g. \cite{chatterjee2005error}.

First, we compute the distance induced by the original process:
\begin{align*}
&\E\left[(\langle x, W x \rangle - \langle x', W x' \rangle + b_*\langle x, Z y \rangle - b_* \langle x', Z y' \rangle)^2\right] \\
&= \E\left[(\sum W_{ij} (x_i x_j - x'_i x'_j))^2\right] + b_*^2 \E\left[(\sum Z_{ij} (x_i y_j - x'_i y'_j))^2\right] \\
&= (4/n) \sum_{i < j} (x_i x_j - x'_i x'_j)^2 + (2/n)\sum_i (x_i - x'_i)^2 +  (b_*^2/p) \sum (x_i y_j - x'_i y'_j)^2 \\
&= (2/n) \sum_{i,j} (x_i x_j - x'_i x'_j)^2 +  (b_*^2/p) \sum (x_i y_j - x'_i y'_j)^2
= (4/n)(1 - \langle x, x' \rangle^2) + (2b_*^2/p)(1 - \langle x, x' \rangle \langle y, y' \rangle).
\end{align*}
For the upper bound process, we have:
\begin{align*}
\E\left[(\langle x - x', g \rangle + \langle y - y', h \rangle)^2\right] 
&= \frac{4 + b_*^2n/p}{n}\|x - x'\|^2 + \frac{b_*^2}{p}\|y - y'\|^2 \\
&=  \frac{4}{n}(2 - 2\langle x, x' \rangle) + \frac{b_*^2}{p}(4 - 2 \langle x, x' \rangle - 2 \langle y, y' \rangle)  
\end{align*}
so the latter minus the former is
\begin{align*} 
\MoveEqLeft (4/n)(1 - 2\langle x, x' \rangle + \langle x, x' \rangle^2) + (2b_*^2/p)(1 - \langle x, x' \rangle - 1 \langle y, y' \rangle + \langle x,x'\rangle\langle y,y'\rangle) \\
&= (4/n)(1 - \langle x, x' \rangle)^2 + (2b_*^2/p)(1 - \langle x, x' \rangle)(1 - \langle y, y' \rangle) \\
&\ge 0 
\end{align*}
which proves the upper bound by Sudakov-Fernique. 

For the lower bound process, we have by a similar calculation to the original process that:
\begin{align*}
\E\left[(\langle x, D x \rangle - \langle x', D x' \rangle + \langle y, E y \rangle - \langle y', E y' \rangle)^2\right] 
&= [4(1 + b_*^2n/4p)/n](1 - \langle x, x' \rangle^2) + [b_*^2/p](1 - \langle y, y' \rangle^2)
\end{align*}
so the difference of the distances of the original process with the lower bound process is
\begin{align*}
(b_*^2/p)[\langle x, x' \rangle^2 - 2\langle x, x' \rangle \langle y, y' \rangle + \langle y, y'\rangle^2] = (b_*^2/p)(\langle x, x' \rangle - \langle y, y'\rangle)^2 \ge 0  
\end{align*}
which proves the lower bound by Sudakov-Fernique. 
\end{proof}

\paragraph{Upper bound summary.}
The argument for upper bound proceeds (Lemma 16) by using that $G$ and $v$ and $H$ and $u$ are nearly orthogonal in high dimensions. Then the problem reduces to a two-dimensional optimization. 

%\fnote{lower bound direction may require some new details, hopefully minor}

\paragraph{Lower bound summary.}
We now go through the lower bound. 
Define $b,\nu$ such that
\begin{equation} 
b_* = b\sqrt{p/n}, \quad \mu = \nu \sqrt{n/p}
\end{equation}
so the lower bound optimization from Lemma~\ref{lem:prop13} is
\begin{equation*}
 \max_{x \in S_n, y \in S_p} \left[\frac{\lambda}{n} \langle x, v \rangle^2 + \langle x, D  x\rangle + b\sqrt{\frac{\nu \sqrt{p/n}}{n}} \langle x, v \rangle \langle y, u \rangle + \langle y, E y \rangle  \right]    
\end{equation*}
where $D_{ij} \sim N(0, (1 + b^2/4)/n)$ for $i < j$ and $D_{ii} \sim N(0, 2(1 + b^2/4)/n)$ is a symmetric random matrix, and $E_{ij} \sim N(0, b^2p/4n)$ and $E_{ii} \sim N(0, b^2p/2n)$. Observe by the equality case of the AM-GM inequality that
\begin{align*}
&\max_{x \in S_n, y \in S_p} \left[\frac{\lambda}{n} \langle x, v \rangle^2 + \langle x, D  x\rangle + b\sqrt{\frac{\nu \sqrt{p/n}}{n}} \langle x, v \rangle \langle y, u \rangle + \langle y, E y \rangle  \right]  \\
&= \max_{x \in S_n, y \in S_p} \min_{t \ge 0} \left[\frac{\lambda}{n} \langle x, v \rangle^2 + \langle x, D  x\rangle + \frac{b \nu t}{2n}\langle x, v \rangle^2 + \frac{b\sqrt{p/n}}{2 t} \langle y, u \rangle^2 + \langle y, E y \rangle  \right]  \\   
&= \max_{x \in S_n, y \in S_p} \min_{t \ge 0} \left[ \langle xx^T, D + \frac{\lambda + b\nu t/2}{n} vv^T  \rangle + \langle yy^T, E + \frac{b\sqrt{p/n}}{2 t} uu^T \rangle  \right]  \\
&= \max_{x \in S_n, y \in S_p} \min_{t \ge 0} \left[ \langle xx^T, D + \frac{\lambda + b\nu t/2}{n} vv^T  \rangle + \langle yy^T, E' + \frac{1}{2 t} uu^T \rangle b \sqrt{p/n}  \right]
\end{align*}
where $E' = E \sqrt{n/pb^2}$ so $E'_{ij} \sim N(0,1/4)$ and $E'_{ii} \sim N(0,1/2)$.

Define
\[ G(\kappa,\sigma^2) := \begin{cases}
\kappa/2 + \sigma^2/2\kappa & \text{if $\kappa^2 \ge \sigma^2$} \\
\sigma & \text{otherwise}
\end{cases}\]
and recall
\begin{thm}[Theorem ? of \cite{?}]

\end{thm}
TODO. We need to compute value of the optimization up to $o(1)$ terms and also worry about concentration to see how small we can take $p$. Need to use precise results on max eigenvalue fluctuations? Maybe we just need to pick $b$ differently than they did. (They picked $b$ constant I think, but looks like we want growing with $n$?)

\paragraph{alternative approach?}
Could try to directly look at the matrix
\begin{align*} 
M(\xi) 
&:= A + \frac{2\mu^2p^2}{\lambda^2n^2\xi} B B^T + \frac{\xi}{2} I_n \\
&= \frac{\lambda}{n} vv^T + W + \frac{2\mu^2p^2}{\lambda^2n^2\xi}\left[(\mu/n) vv^T + \sqrt{\mu/n}[vu^TZ^T + Z uv^T] + ZZ^T \right] + \frac{\xi}{2} I_n 
\end{align*}
maybe it becomes easier to analyze directly when $p/n = o(1)$? How to heuristically see the threshold from this expression? Note that $(1/n) Z^TZ \approx I_p/p$ by Wishart concentration, so the eigenvalues of $ZZ^T$ are size $n/p$. Based on this a more naive idea is to take
\[ A + c(p/n) B B^T = \frac{\lambda}{n} vv^T + W + \frac{c\mu p/n}{n} vv^T + \cdots \]
and if we ignore the other contributions, it would give a threshold of $\lambda + c\mu p/n > 1$ which doesn't really look right. Maybe a better heuristic is to consider
\[ \frac{\lambda}{n} vv^T + W + K[v\sqrt{\mu/n}  + Zu][v\sqrt{\mu/n} + Zu]^T] + ? \approx \frac{\lambda}{n} vv^T + W + \frac{K\mu}{n} vv^T + K\sqrt{\mu/pn}[gv^T + vg^T] + \cdots  \]
and since the last term is roughly size $K\sqrt{\mu}$ it suggests taking $K$ constant? That doesn't make sense either.

The equation can be interpreted as 
\[ \lambda^2 n/p + \mu^2 > n/p \]
could we get something by restricting everything to the span of $(1/n) Z^T Z$? The size of $W$ in this space is only $p/n$ instead of constant size which explains the ``boost'' from $\lambda$ to $\lambda\sqrt{n/p}$? But restricted to that subsppace, unclear if $A$ is useful at all...
\iffalse
HEURISTIC. Seems like when $p/n \to 0$ and we choose $b$ as in their paper, we can simplify optimization by dropping $E'$ and get
\begin{align*}
&\max_{x \in S_n, y \in S_p} \min_{t \ge 0} \left[ \langle xx^T, D + \frac{\lambda + b\nu t/2}{n} vv^T  \rangle + \langle yy^T, \frac{b}{2 t} uu^T \rangle \sqrt{p/n}  \right] \\
&=\max_{x \in S_n} \min_{t \ge 0} \left[ \langle xx^T, D + \frac{\lambda + b\nu t/2}{n} vv^T  \rangle + \frac{b}{2 t}  \sqrt{p/n}  \right] 
\end{align*}
and then taking $t = o(1)$ very slowly, only the first term remains? Probably have a missing scaling factor somewhere. Check $\lambda = 0, \mu = 0$ case. Perhaps the optimal tuning of $b$ should be different.
\fi

==> packages_colt.tex <==
\usepackage{mathtools}
\usepackage{bbm}

